A Decade of Mal-Activity Reporting: A Retrospective Analysis of Internet Malicious Activity Blacklists

This paper focuses on reporting of Internet malicious activity (or mal-activity in short) by public blacklists with the objective of providing a systematic characterization of what has been reported over the years, and more importantly, the evolution of reported activities. Using an initial seed of 22 blacklists, covering the period from January 2007 to June 2017, we collect more than 51 million mal-activity reports involving 662K unique IP addresses worldwide. Leveraging the Wayback Machine, antivirus (AV) tool reports and several additional public datasets (e.g., BGP Route Views and Internet registries) we enrich the data with historical meta-information including geo-locations (countries), autonomous system (AS) numbers and types of mal-activity. Furthermore, we use the initially labelled dataset of approx 1.57 million mal-activities (obtained from public blacklists) to train a machine learning classifier to classify the remaining unlabeled dataset of approx 44 million mal-activities obtained through additional sources. We make our unique collected dataset (and scripts used) publicly available for further research. The main contributions of the paper are a novel means of report collection, with a machine learning approach to classify reported activities, characterization of the dataset and, most importantly, temporal analysis of mal-activity reporting behavior. Inspired by P2P behavior modeling, our analysis shows that some classes of mal-activities (e.g., phishing) and a small number of mal-activity sources are persistent, suggesting that either blacklist-based prevention systems are ineffective or have unreasonably long update periods. Our analysis also indicates that resources can be better utilized by focusing on heavy mal-activity contributors, which constitute the bulk of mal-activities.

==> files/geo_asn_lvl_analysis.tex <==
In Table~\ref{tab:dataset}, we observe that on average 51 IPs that involved in malicious activity in 12,948 unique ASes. We also note that on average 3,345 IPs, involved in Mal-activities, in almost every country in the world. In this section, we analyze whether the IPs (resp. volume and AV-Score of Mal-Activities) in our dataset are evenly distributed amongst ASes and countries. We analyze the hosting infrastructures and geolocations of  malicious activities in our dataset. %Our analysis aim to answer essential questions: What are the geo-diversity and geo-density (classes) of malicious activities? Are (classes of) malicious activities concentrated at particular hosting infrastructure? What is the AV-Score of prominent geolocations and hosting infrastructures? 

To measure the volume of (categories of ) Mal-Activities per AS, we use BGP route-review dataset to extract an ASN of given IP that involved in Mal-Activity. For each AS, we measure its average AV-Score by averaging the maximum AV-Scores of IPs that belong to it. Similarly, using of MaxMind dataset~\cite{maxmind} and Potaroo datasets (cf. \S~\ref{sec:data_augmentation}), we map each IP to its geolocation (i.e., hosting country). To determine the AV-Score of activities originated from a country, we average the maximum AV-Scores of IPs per country. 
% AS-Level Analysis

\subsection{AS-Level Analysis} 
\label{subsec:infrastructure}
%
%We investigate the volume of (class of ) malicious activities per AS. We use BGP route-review dataset to extract an ASN that correspond to a given IP in our dataset. For each AS, we measure its average AV-Score by averaging the maximum AV-Score of IP addresses that belong to it.
%
{\bf Volume of Mal-Activities per AS.} Figure~\ref{vt:cc:vol:avscore} show the distribution of volume and AV-Score of Mal-Activities per AS. We observe that 18\% of the ASes involved in only malicious activity while 60\% of the total contributed to at least 5 malicious activities. Among the different classes of malicious activities, we observe Fraudulent Services, Phishing, and Malware have the first, second, and third, respectively, volume of malicious activities per AS. On the other hand, Spammers class of malicious activities have the least volume per AS. Interestingly, the CDFs depicted in Figure~\ref{Fig:results:asc_avscore_cdf} suggest that the ASes that correspond to Spammers and PUP--both have relatively lower volumes--are more malicious when compared to the rest of the classes. 80\% of PUP's ASes have AV-Score at least 40\% while 20\% of Spammers' ASes have AV-Score at most 18\%. 

Based on the volume of malicious activities, we rank the top-10 ASes in Table~\ref{tab:asn:geodiversity}. We notice that AS16509 (belong to AMAZON-02 and located in US) has AV-Score 85\% and is the most aggressive in term of volume of malicious activities. We also observe that it has contributed to all classes of malicious activities, predominantly to Malware (658K, 86\%), Phishing (436K, 84\%), and PUP (265K, 81\%). 


\begin{figure}[ht!]
\centering
%\subfloat[\small Volume]{\includegraphics[width=0.50\columnwidth]{plots/asn_attack_cdf.pdf}\label{Fig:results:attk_prob_cdf:ASN}}
\subfloat[\small Volume]{\includegraphics[width=0.50\columnwidth]{markered_plots/asn_attack_cdf-crop.pdf}\label{Fig:results:attk_prob_cdf:ASN}}
\subfloat[\small AV-Score]{\includegraphics[width=0.50\columnwidth]{markered_plots/asn_average_av_rank-crop.pdf}\label{Fig:results:asc_avscore_cdf}}
\vspace{-0.45cm}
\caption{\small Volume and AV-Score of Mal-Activities per AS. } 
\vspace{-0.5cm}
\label{vt:cc:vol:avscore}
\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.99\columnwidth]{plots/asn_attack_cdf.pdf}
%\caption{Here, cumulative distribution of Volume of malicious activities  per ASN.}
%%\ik{Fill Table~\ref{tab:geodiversity} with TOP-10 countries as per volume. Include the average VT-score per geo-location with standard deviation.} } 
%\label{Fig:results:attk_prob_cdf:ASN}
%\end{figure}
%
%\begin{figure}[H]
%\centering
%\includegraphics[width=0.99\columnwidth]{plots/eplots/asn_attack_av_rank.pdf}
%\caption{Here, cumulative distribution of AV-Score per AS.  } 
%\label{Fig:results:asc_avscore_cdf}
%\end{figure}


\begin{table}[ht!]
\centering
%\scriptsize
\Small
\tabcolsep=0.04cm
\resizebox{0.83\textwidth}{!}{\begin{minipage}{\textwidth}
\begin{tabular}{rrrrrrrrrrrrrrrrrr } 
\toprule
& &    \multicolumn{2}{c}{\bf Malware} & \multicolumn{2}{c}{\bf Phishing}& \multicolumn{2}{c}{\bf Spam.}& \multicolumn{2}{c}{\bf Exploits}& \multicolumn{2}{c}{\bf PUP}& \multicolumn{2}{c}{\bf FS}& \multicolumn{2}{c}{\bf Total}\\
ASN	& Org.	& Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	\\
\midrule
16509 &Amazon, Inc., US	&	658K	&	86\%	&	436K	&	84\%	&	45	&	86\%	&	20K	&	87\%	&	265K	&	81\%	&	26K	&	72\%	&	1.4M	&	85\%	\\
14618&Amazon, Inc., US	&	251K	&	72\%	&	65K	&	66\%	&	107	&	98\%	&	30K	&	70\%	&	100K	&	74\%	&	19K	&	75\%	&	465K	&	71\%	\\
20940&Akamai, US	&	48K	&	79\%	&	270K	&	80\%	&		&		&	1K	&	75\%	&	33K	&	81\%	&	942	&	64\%	&	353K	&	79\%	\\
26496&GoDaddy, LLC, US	&	184K	&	78\%	&	37K	&	77\%	&	71	&	82\%	&	8K	&	89\%	&	1K	&	84\%	&	106K	&	81\%	&	336K	&	79\%	\\
4134 & ChinaNet, CN		&	26K	&	60\%	&	138K	&	80\%	&		&		&	1K	&	71\%	&	488	&	71\%	&	2K	&	18\%	&	168K	&	78\%	\\
%13335	&	54K	&	48\%	&	20K	&	59\%	&	90	&	79\%	&	2K	&	60\%	&	5.5K	&	55\%	&	65K	&	38\%	&	147K	&	50\%	\\
%209		&	13K	&	84\%	&	113K	&	81\%	&	54	&	97\%	&	518	&	84\%	&	9K	&	90\%	&	454	&	84\%	&	136K	&	82\%	\\
%2914		&	21K	&	81\%	&	87K	&	81\%	&		&		&	406	&	81\%	&	13K	&	85\%	&	158	&	78\%	&	122K	&	81\%	\\
%35994	&	17K	&	82\%	&	82K	&	81\%	&		&		&	319	&	75\%	&	11K	&	84\%	&	158	&	67\%	&	111K	&	80\%	\\
\bottomrule
\end{tabular}
 \end{minipage}}
\caption{\small Top 5 ASes with Volume (Vol.) of malicious activities and the average AV-score (AVS.). }
\label{tab:asn:geodiversity}
\vspace{-0.8cm}
\end{table}


To further investigate the contributions of ASes to different classes of malicious activities, we measure Specialization. In Figure~\ref{Fig:results:attk_cdf}, we observe that 45\% of ASes participated in only one class of malicious activities while 5\% of them involved in all six classes. We also measure the ASes' affinity to malicious activities. The affinity of ASes to different classes are:  PUP (0.366), Fraudulent Services (0.626), Malware (0.543), Exploits (0.561), Phishing (0.458), and Spammers (0.714). The comparatively large affinity ASes to Spammers suggests that spamming activities evenly distributed amongst the ASes while the small values of ASes for PUP indicates that a subset of ASes aggressively contributing to PUP activities. Our comparison of IPs' affinity for PUP (0.871, cf. Section~\ref{subsec:ip_specialization}), further suggest that offenders use multiple IPs from same  AS to inflict PUP class of malicious activities. On the other hand, abusers that inflict Spammers class of malicious activities choose IPs from diverse set of ASes. 
%\ik{Include the stake-bar plot for the X\% of the volume of ASNs.}

%\begin{table}[h!]
%\centering
%\scriptsize
%\begin{tabular}{ rrrrrrrr }
%\toprule
%\toprule
%{\bf Metric} & {\bf PUP} & {\bf FS} & { \bf Malware}&{\bf Exploits}&{\bf Phishing} &{\bf Spammers}&{\bf Total}\\
%\midrule
%Affinity &  0.366	&	0.626	&	0.543	&	0.561	&	0.458	&	0.714	&	0.513	\\
%%Speci. &     	0.0493 &      	0.0675	& 	0.614 &	0.0265 & 	0.0888&     	0.00211&	0.152\\
%\bottomrule
%\end{tabular}
%\caption{Affinity of ASes. \ik{Update this with new values}}%The affinity of the reports within an attack type over the contributing ASNs. Here UL represent ``unlabelled'' malicious activities (see. Table~\ref{tab:dataset}) in our dataset. \ik{As we can mention these numbers in text, perhaps, we should kick this table out. Suggestions?}}
%\label{tab:asn_affinity_purity}
%\vspace{-0.4cm}
%\end{table}



%\ben{Figure \ref{Fig:results:host_degree} displays the CDF of Host components with respect tot he number of attack classes it has participated within.}
% -Ben.Z Moved image further up in section
%\begin{figure}[t!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/host_degree.pdf}
%\caption{CDF of the Degree of Attack Type Participation (number of classes it has participated in) in the various tiers of Hosting Infrastructure} 
%\label{Fig:results:host_degree}
%\end{figure}



%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{plots/asn_counts.pdf}
%\caption{ASN Distribution of Reported Malware. \ben{asn\_counts.py}  \ik{Normalize vertical axis and reveal  the distribution (long-tail or not).}}
%\label{fig:asn_freq}
%\end{figure}

%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{plots/asn_counts_v2.pdf}
%\caption{ASes distribution involved in malicious activities. Here, inset 1 and inset 2 show the middle and tail of distribution, respectively. The $x$-axis show the AS number (i.e., ASN). \ik{@Ben: Normalize vertical axis and replot this.}}% rank on inset x-axis \ben{asn\_counts\_v2.py}  \ik{@Ben: Normalize vertical axis and replot this.}}
%\label{fig:asn_freq}
%\end{figure}


%We answer these questions in the following subsections. 
\subsection{Geodiversity of Mal-Activities}
\label{subsec:gdistribution}
%Using of MaxMind dataset~\cite{maxmind} and Potaroo datasets (cf. \S~\ref{sec:data_augmentation}), we map each IP to its geolocation (i.e., hosting country). To determine the AV-Score of activities originated from a country, we average the maximum AV-Scores of IPs per country.





%Figure~\ref{fig:no_attack_cls} shows the distribution of number of attacks per country. We observe only one type of attacks in 25\% of the countries with 94\% of the countries such as Swaziland and Haiti have malicious activities that belong to malware class while the remaining 6\% of the countries such as Saint Vincent and Northern Mariana Islands have sources that belong to phishing attack class. Similarly, at least 54\% of the countries such as US and Russia source malicious activities that belong to more than three different attack classes. 

\textbf{Volume of Mal-Activities per County. } 
First, we analyze the frequency (classes) of malicious activities per country both as CDFs (Figure~\ref{Fig:results:country_attack_cdf}) and as a Table~\ref{tab:geodiversity}. The distributions depicted by the CDF show that classes of malicious activities are drastically different from one class to another. In fact, the red curve representing Malware is relatively flat indicating that this phenomena is prevalent and originating from most of the countries. In the other hand, spamming bots (i.e., spammers class of malicious activities) are concentrated in few countries. 
%
Moreover, we observe 4\% of the countries have only malicious activities. Interestingly, 82\% of countries have more than one malicious activities of class Spammers which is relatively lower when compared to other classes. Overall, 20\% of countries have at least 10K malicious reports. 
\begin{figure}[ht!]
\centering
\vspace{-0.6cm}
\subfloat[\small Volume]{\includegraphics[width=0.50\columnwidth]{new_plots/cc_attack_cdf.pdf}\label{Fig:results:country_attack_cdf}}
\subfloat[\small AV-Score]{\includegraphics[width=0.50\columnwidth]{new_plots/cc_attack_av_rank.pdf}\label{Fig:results:country_avscore_cdf}}
\vspace{-0.45cm}
\caption{\small Volume and AV-Score of Mal-Activities per country.} 
\vspace{-0.4cm}
\label{vt:cc:vol:avscore}
\end{figure}

\textbf{AV-Score of Mal-Activities per County. } Figure~\ref{Fig:results:country_avscore_cdf} the AV-Score of malicious activities per country. We observe 95\% of countries have malicious activities with AV-Score at least 3\%. We determine that PUP per country is the most malicious according to our AV-Score with 80\% of the countries have AV-Score at least 87\% (i.e., 56 AV-Tools flagged activities as malicious). 

Based on the volume and AV-score of malicious activities, we rank the top-10 countries in Table~\ref{tab:geodiversity}. We observe that 4.7M malicious activities (AV-score 79\%) with predominant Malware (2M) and Phishing (1.6M) originated from US. Similarly, besides sourcing Malware (94K), Russia is contributing more to Fraudulent Services (62.5K with AV-Score 98\%) when compare to other classes, however, with relatively lower average AV-Score, 47\%. Even though, Virgin Islands, British (VG) is ranked 8$^{th}$ in term of volume of malicious activities,  we determine that the activities originated from VG have the highest average AV-Score (94\%). %In fact, while the malware class is distributed nearly evenly among the top 10 countries, other malicious classes are targeting (or the home for) few countries.  

%\ik{Include the stake-bar plot for the X\% of the volume of countries.}
%Next, we show the frequency of malicious activities per attack class per country in Figure~\ref{fig:attack_occurances} and present the frequency of malicious activities in heatmap i.e., Figure~\ref{fig:country_attk_freq}. In term of number occurrences and geographical diversity, the malware attack class is more aggressive and prevalent while Spamming attack is the least one. We observe that 60\% of the countries have at least 100 malware activities. The US sources malicious activities of all attack class except spamming activities. This indicates that just because a country has many occurrences, it may still source a particular kind of attack, this is not only applicable for the right hand side of the heatmap, as we move left the gradient of the cells do not decrease sequentially, with the occurrences for a particular attack increasing and decreasing while moving left. We further investigate the attacks' geo-diversity by performing temporal analysis in Section~\ik{xref}. 

\begin{table}[ht!]
\centering
%\scriptsize
\Small
\tabcolsep=0.04cm
\begin{tabular}{rrrrrrrrrrrrrrr}
\toprule
 & \multicolumn{2}{c}{\bf Malware} & \multicolumn{2}{c}{\bf Phishing}& \multicolumn{2}{c}{\bf Spam.}& \multicolumn{2}{c}{\bf Exploits}& \multicolumn{2}{c}{\bf PUP}& \multicolumn{2}{c}{\bf FS}& \multicolumn{2}{c}{\bf Total}\\
CC	&	Vol. 	&	AVS.	&	Vol. 	&	AVS.	&	Vol. 	&	AVS.	&	Vol. 	&	AVS.	&	Vol. 	&	AVS.	&	Vol. 	&	AVS.	&	Vol. 	&	AVS	\\
\midrule
US	&	2M	&	77\%	&	1.6M	&	79\%	&	3K	&	92\%	&	602K	&	80\%	&	100K	&	83\%	&	450K	&	73\%	&	4.7M	&	79\%	\\
CN	&	56K	&	65\%	&	308K	&	79\%	&	249	&	96\%	&	3K	&	80\%	&	4K	&	75\%	&	8K	&	37\%	&	380K	&	78\%	\\
DE	&	90K	&	71\%	&	105K	&	77\%	&	364	&	80\%	&	14K	&	77\%	&	7K	&	71\%	&	35K	&	67\%	&	252K	&	74\%	\\
RU	&	94K	&	61\%	&	18K	&	69\%	&	1K	&	75\%	&	2K	&	39\%	&	9K	&	59\%	&	63K	&	23\%	&	186K	&	47\%	\\
FR	&	68K	&	72\%	&	34K	&	67\%	&	121	&	81\%	&	8K	&	82\%	&	17K	&	73\%	&	26K	&	65\%	&	153K	&	70\%	\\
%UA	&	104K	&	55\%	&	12K	&	71\%	&	239	&	28\%	&	443	&	50\%	&	5K	&	37\%	&	8K	&	20\%	&	129K	&	57\%	\\
%NL	&	59K	&	69\%	&	22K	&	76\%	&	253	&	87\%	&	7K	&	77\%	&	5K	&	76\%	&	22K	&	59\%	&	116K	&	72\%	\\
%VG	&	51K	&	94\%	&	9K	&	88\%	&	642	&	97\%	&	1K	&	96\%	&	10K	&	91\%	&	16K	&	94\%	&	88K	&	94\%	\\
%GB	&	45K	&	58\%	&	16K	&	64\%	&	179	&	87\%	&	3K	&	73\%	&	3K	&	54\%	&	15K	&	45\%	&	82K	&	58\%	\\
%PL	&	43K	&	65\%	&	4K	&	62\%	&	11	&	66\%	&	221	&	68\%	&	460	&	69\%	&	8K	&	26\%	&	56K	&	59\%	\\
\bottomrule
\end{tabular}
\caption{\small Top 5 countries with Volume (Vol.) of malicious activities and the average AV-score (AVS.). }%FS and CC represent fraudulent services (a class of malicious activities) and country code, respectively.}%  \ik{TODO: For each cell, include the AVS.}}
\vspace{-0.9cm}
\label{tab:geodiversity}
\end{table}


%\ik{Include the stake-bar plot for the X\% of the volume of Countries.}

%\begin{table}[ht!]
%\centering
%\scriptsize
%\begin{tabular}{ rrrrrrrr }
%\toprule
%\midrule
%{\bf Metric} & {\bf PUP} & {\bf FS} & { \bf Malware}&{\bf Exploits}&{\bf Phishing} &{\bf Spammers}&{\bf Total}\\
%\midrule
%Affinity & 0.105& 	0.437& 	0.367& 	0.451	& 	0.249& 	0.556& 	0.319\\
%%Speci. &	0.00328 &	0.0558&	0.711&	0.0221&	0.0706&	0.00148&	0.135\\
%\bottomrule
%\end{tabular}
%\caption{Affinity of countries. }%The affinity of the malicious activities and contributing geolocation specialization.  Here UL represent ``unlabelled'' malicious activities (see. Table~\ref{tab:dataset}) in our dataset. \ik{As we can mention these numbers in text, perhaps, we should kick this table out. Suggestions?}}
%\label{tab:cc_affinity_purity}
%\vspace{-0.4cm}
%\end{table}

%In Table~\ref{tab:cc_affinity_purity}, we show the affinity of countries that originate malicious activities. 
\textbf{Specialization and Affinity of Countries. }  In Figure~\ref{Fig:results:attk_cdf}, we notice that 80\% of countries contributes to more than one class of malicious activities. We observe that 20\% of countries host only Malware class of malicious activities, while 27\% (54) host all six malicious classes. 

Moreover, we measure the affinities of countries that originate malicious activities. Affinities of countries per class of malicious activities are: PUP (0.105), Fraudulent Service (0.437), Malware (0.367), Exploits (0.451), Phishing (0.249), and Spammers (0.556). %& 	0.319\\
The affinity of countries to all malicious activities is 0.319 which is 0.5 smaller than the affinities of IPs (see Section~\ref{subsec:ip_specialization}). This suggests that the number of malicious activities are unevenly distributed among the countries i.e., a subset of countries contributing most of the malicious activities. When we compare the classes of malicious activities, we determine that Spammers (0.556) has the largest affinity followed by Exploits (0.451) and Fraudulent services (0.437). Comparing the countries' affinities with IP addresses' affinities (see Section~\ref{subsec:ip_specialization}) reveal some interesting observations: As PUP has countries' affinity 0.105 which is smaller than its IPs affinity (0.871) by 0.766, suggesting at country-level a subset of countries contributing to PUP. 



%\textbf{Malicious Activities per City. }
%Next, we drill-down to analyze volume of malicious activities per city.  %To determine the AV-Score of activities originated from a city, we average the maximum AV-Scores of IPs that belong to the city. 
%We show the result of our analysis in Figure~\ref{Fig:results:city_attack_cdf}. The distribution suggests that 40\% of the cities have at least 10 malicious activities with 66\% of them involved in Malware class of malicious activities. We observe that all other classes of malicious activities  follow similar trends. Similar to AV-Score of malicious activities per country (cf. Figure~\ref{Fig:results:country_avscore_cdf}), We observe that PUP class of malicious activities are relatively more malicious when compared to the rest of the classes. 60\% of the countries have malicious activities (of class PUP) with AV-Score 95\%.  
%
%We analyze the long-tail of the distributions, in Figure~\ref{Fig:results:city_attack_cdf}, to further analyze the cities with high volume of malicious activities. Table~\ref{tab:citydiversity} ranks the top-10 by volume and AV-Score. We notice that Seattle and Ashburn are the first and second most contributors to Malware class of malicious activities with AV-Score 88\% and 78\%, respectively. Combridge is unevenly sourcing Phishing (with Vol.=358K and AV-Score=78\%) while Scottsdale is originating in Fraudulent Services (101K, 82\%) .  
%
%We determine the affinity of cities that originate classes of malicious activities. The affinities are: PUP (0.358), Phishing (0.474), Malware (0.466), Exploits (0.514), FS (0.55),  Spammers (0.693). The smaller affinity of PUP suggests that the number of malicious activities are unevenly distributed among the cities i.e., a subset of cities are contributing most of the PUP class of malicious activities. When we compare the classes of malicious activities, we determine that cities are relatively evenly contributing to Spammers class of malicious activities. 
%
%In Figure~\ref{Fig:results:attk_cdf}, we notice that 24\% of cities contribute to more than one class of malicious activities. We further investigate that \red{XX\%} of cities host only Malware, \red{xx\%} Spammers, and \red{yy\%} PUP class of malicious activities, while XX\% (54) host all six malicious classes. 
%
%\begin{figure}[ht!]
%\centering
%%\subfloat[\small Volume]{\includegraphics[width=0.50\columnwidth]{plots/cities_attack_cdf.pdf}\label{Fig:results:city_attack_cdf}} % Old plot
%\subfloat[\small Volume]{\includegraphics[width=0.50\columnwidth]{new_plots/city_attack_cdf.pdf}\label{Fig:results:city_attack_cdf}} % new plot
%\subfloat[\small AV-Score]{\includegraphics[width=0.50\columnwidth]{new_plots/city_attack_av_rank.pdf}\label{Fig:results:city_avscore_cdf}}
%\caption{CDFs of number of malicious activities (Volume) and AV-Score per city.  Table~\ref{tab:citydiversity} highlight the top-10 Cities.} 
%%\vspace{-0.7cm}
%\label{vt:city:vol:avscore}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.99\columnwidth]{plots/cities_attack_cdf.pdf}
%\caption{Here, cumulative distribution of Volume of malicious activities per city. \ik{TODO: replace Occurence by ``Volume of malicious activities per city''.}.  Table~\ref{tab:geodiversity} to highlight the top-10 cities.}% \ben{For every plot of this type we have 2 different skews, the current skew includes all infrastructure components from the larger dataset, so we can compare between the categories on the y-axis, however for the smaller attack groups, they get dwarfed by the more populous ones. Instead we can do it as a CDF over the non-zero set of infrastructure components which will show the y-axis distribution for these smaller attacks much more clearly.}} 
%\label{Fig:results:city_attack_cdf}
%\end{figure}
%
%\begin{figure}[H]
%\centering
%\includegraphics[width=0.99\columnwidth]{plots/eplots/city_attack_av_rank.pdf}
%\caption{Here, cumulative distribution of AV-Score per City. } 
%\label{Fig:results:city_avscore_cdf}
%\end{figure}

%
%\begin{table}[ht!]
%\centering
%\scriptsize
%%\Small
%\tabcolsep=0.04cm
%\begin{tabular}{rrrrrrrrrrrrrrr}
%\toprule
% &  \multicolumn{2}{c}{\bf Malware} & \multicolumn{2}{c}{\bf Phishing}& \multicolumn{2}{c}{\bf Spam.}& \multicolumn{2}{c}{\bf Exploits}& \multicolumn{2}{c}{\bf PUP}& \multicolumn{2}{c}{\bf FS}& \multicolumn{2}{c}{\bf Total}\\
%Cities	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	\\
%\midrule
%Seattle	&	452K	&	87\%	&	218K	&	89\%	&		&		&	16K	&	83\%	&	242K	&	90\%	&	16K	&	84\%	&	943K	&	88\%	\\
%Ashburn	&	425K	&	79\%	&	194K	&	79\%	&	138	&	96\%	&	33K	&	75\%	&	116K	&	73\%	&	22K	&	76\%	&	789K	&	78\%	\\
%Cambridge	&	73K	&	81\%	&	358K	&	78\%	&	8	&	96\%	&	2K	&	84\%	&	59K	&	71\%	&	4K	&	88\%	&	495K	&	78\%	\\
%Scottsdale	&	178K	&	79\%	&	36K	&	77\%	&	70	&	82\%	&	7K	&	85\%	&	1K	&	90\%	&	101K	&	82\%	&	323K	&	80\%	\\
%Mountain View	&	38K	&	86\%	&	108K	&	81\%	&	241	&	88\%	&	1K&	88\%	&	25K	&	90\%	&	12K	&	82\%	&	185K	&	83\%	\\
%%San Francisco	&	62K	&	52\%	&	22K	&	60\%	&	42	&	42\%	&	2K	&	59\%	&	6,K	&	59\%	&	69K	&	47\%	&	161K	&	54\%	\\
%%Boardman	&	54K	&	72\%	&	85K	&	76\%	&	1	&	13\%	&	1K	&	69\%	&	13K	&	80\%	&	7K	&	50\%	&	160K	&	74\%	\\
%%New York	&	30K	&	89\%	&	18K	&	80\%	&	91	&	95\%	&	1K	&	95\%	&	56K	&	93\%	&	20K	&	85\%	&	126K	&	89\%	\\
%%Englewood	&	21K	&	80\%	&	91K	&	81\%	&	4	&	98\%	&	330	&	81\%	&	9K	&	84\%	&	306	&	62\%	&	121K	&	81\%	\\
%%Los Angeles	&	56K	&	72\%	&	16K	&	66\%	&	510	&	96\%	&	8K	&	94\%	&	2K	&	75\%	&	35K	&	77\%	&	118K	&	74\%	\\
%\bottomrule
%\end{tabular}
%\caption{Top 5 cities with Volume (Vol.) of malicious activities and the average AV-score (AV-S). }
%\label{tab:citydiversity}
%%\vspace{-0.6cm}
%\end{table}



==> files/ip_lvl_analysis.tex <==
\label{sec:domainip}
We first define the three metrics in use and then begin with analyzing the spatial distribution of Mal-Activities and the prevalence of Mal-Activities per IP addresses in our dataset. Then we quantify the IP addresses' participation in different classes of malicious activities. 

\subsection{Metrics in use}
\label{sec:metrics}
To better understand how Mal-Activities are distributed amongst IPs, ASes and Geolocations, we first introduce two diversity (or a homogeneity) metrics named \emph{Affinity} and \emph{Specialization} by adopting \textit{Shannon entropy}. Then, we introduce \emph{AV-score} that quantifies the prevalence of Mal-Activities of IPs among many Anti-Virus scanners and databases. %These three metrics are used throughout the paper for retrospective spatiotemporal analysis of Mal-Activity distribution.

{\bf Affinity.} To measure the spread of a given class of Mal-Activities (cf. \S~\ref{sec:mtypes}) across reported malicious Hosts, we define \emph{Affinity} as normalized Entropy per Mal-Activity $a$ as $A(a) = (-\sum_{\forall h} P(h) \log_2{P(h)})/\log_2 k$ where;
\begin{equation} \label{eqn:attack_affinity}
P(h) = \frac{\# \, \text{of reports from host $h$ with activity $a$}}{\text{Total} \, \# \, \text{of reports for activity $a$}}
\end{equation}
In this regard, $A(a)=1$ represents that reports of Mal-Activity $a$ are evenly distributed among all hosts and conversely $A(a)=0$ represents that all reports are concentrated on a single host. 

{\bf Specialization.} The distribution of hosts across classes of Mal-Activities is defined as normalized Entropy per host $h$ as  $S(h) = (-\sum_{\forall a} P(h) \log_2{P(h)})/\log_2 k$ where the probability $P(h)$ is defined as: %in Equation ~\ref{eqn:attack_affinity}. 
\begin{equation} \label{eqn:attack_affinity}
P(h) = \frac{\# \, \text{of reports from host $h$ with activity $a$}}{\text{Total} \, \# \, \text{of reports for host $h$}}
\end{equation}
Strong specialization of hosting one particular Mal-Activity class is represented by higher $S(h)$ value for a given host $h$.

%A(a) = (-\sum_{\forall h} P(h) \log_2{P(h)})/\log_2 k$ 

{\bf AV-score.}
It is imperative to rely on multiple AV scanners and databases to filter Mal-Activities as they often attempt to circumvent certain AV tools and also to reduce false positives~\cite{6234407}. Furthermore, having flagged by multiple AV scanners is an indication of prevalence of the malicious activity. We define \emph{AV-score} to quantify the ``maliciousness'' of an activitiy such that $\text{AV-score}(h) = (\sum_{i=1}^{N}\mathcal{P}_i)/{N}$ where $\mathcal{P}_i$ equals $1$ if an AV tool, $i$, flags a given host $h$ as malicious, otherwise $\mathcal{P}_i$ equals $0$. $N$ is the total number of available AV-tools %\footnote{As of May 15$^{th}$,  2017, VirusTotal used 68 different AV-tools to check malicious activities.} 
used by VirusTotal to determine Mal-Activities of a host.

\subsection{Volume and AV-Score Analysis}  For each IP in our dataset, we measure the number of Mal-Activities (i.e., volume) it involved and maximum AV-Score (see Section~\ref{sec:metrics}) according to VirusTotal.
%
%For a given IP in our dataset, we measure the volume of malicious activities and, %the VT-score. %From VirusTotal dataset, we obtain the number of positives that correspond to URLs on domains. Similarly, 
%from VirusTotal dataset, we obtain the maximum number of malware positives for each domain, referrer, and malicious file (cf. Section~\ref{sec:data_augmentation}). 
As the maximum number of malware positives determines the majority {\it agreement (voting)} amongst AV tools, therefore, we choose the maximum AV-Score to determine the maliciousness of a given IP address. % is that % that correspond to the IP address.

Figure~\ref{vt:ips:vol} shows the distribution of number Mal-Activities per IP in our dataset. We observe that 60\% of IP addresses involved in only one Mal-Activity. Compared to the total IP addresses, 81\% Fraudulent Services' IPs involved in more than one malicious activities. This suggests that a relatively high fraction of Mal-Activities of Fraudulent Services originate from these 81\% of IPs i.e.,  these IPs relatively more ``active'' in term of number of Mal-Activities. Similarly, 44\% of PUP IP address and 36\% of Spammers IP addresses participated in more than one Mal-Activities. Overall, approximately 12\% of all IPs participated in at least 10 malicious activities with 19\% of the them (i.e, in the long-tail of CDFs) participate in activities that belong to at least 3 different classes (see Section~\ref{sec:mtypes}).

%\ben{You can't obtain this 30\% information from just looking at the graph, how large of the tail are you referring to?, Its 19.1\% of the unique IPs participate in 3 or more attacks.
%1 Degree: 482713, 0.797366630106
%2 Degree: 85305, 0.140910562552
%3 Degree: 25787, 0.0425961042908
%4 Degree: 8798, 0.014532924557
%5 Degree: 2470, 0.00408005497337
%6 Degree: 311, 0.000513723520939}. 

%Table~\ref{tab:ipvolumeavscore} contains the detail analysis of malicious files, urls, domains, and referrers that correspond to IP addresses in our dataset. We find that the average number of malicious URLs per IP is \red{XX $\pm$ STD} with average AV-score equals \red{YY $\pm$ STD}. 

Figure~\ref{vt:ips:av-score}, shows the CDFs of maximum AV-Score of Mal-Activities per IP address in our dataset. We determine that 90\% of all IP addresses have AV-Score at least 3\% i.e., at least four AV-tools reported Mal-Activities that correspond to the IPs. On a closer look, the distributions suggest that IPs that correspond to Spammers have higher AV-Score, 85\% of IPs have AV-Score at least 50\%. While Fraudulent Services' IPs have high volume, we observe that they are relatively less malicious (i.e., lower AV-Score) with 50\% of them have AV-Score at most 58\%. %that belong Potentially Unwanted Program have AV-score $\leq$ 3. 

\begin{figure}[h]
\centering
%\subfloat[\small Volume]{\includegraphics[width=0.50\columnwidth]{plots/ips_volume_cdf.pdf}\label{vt:ips:vol}}
\vspace{-0.5cm}
\subfloat[\small Volume]{\includegraphics[width=0.50\columnwidth]{markered_plots/ip_attack_cdf-crop.pdf}\label{vt:ips:vol}}
\subfloat[\small AV-Score]{\includegraphics[width=0.50\columnwidth]{markered_plots/ip_attack_av_rank-crop.pdf}\label{vt:ips:av-score}}
%\subfloat[\small Malicious files on IPs]{\includegraphics[width=0.25\textwidth,height=0.12\textwidth]{./plots/mplots/ips/detected_download_samples_combined_attacks_mean.pdf}\label{vt:ip:files}}
%\subfloat[\small Malicious \textit{referrers} on IPs]{\includegraphics[width=0.25\textwidth,height=0.12\textwidth]{./plots/mplots/ips/detected_referer_samples_combined_attacks_mean.pdf}\label{vt:ip:referrers}}
\vspace{-0.5cm}
\caption{\small CDFs of number of malicious activities (Volume) and AV-Score per IP . } %Table~\ref{tab:ipvolumeavscore} highlight the top-10 IPs.} 
\vspace{-0.4cm}
\label{vt:ips:vol:avscore}
\end{figure}

%\begin{figure}[H]
%\centering
%\subfigure[]{}
%\subfigure[]{}
%\caption{Cumulative distribution of number of malicious activities (Volume) and AV-Score per IP .  
%Table~\ref{tab:ipvolumeavscore} to highlight the top-10 IPs.} 
%\label{vt:ips:vol:avscore}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.99\columnwidth]{plots/eplots/ip_attack_av_rank.pdf}
%\caption{Here, cumulative distribution of AV-Score per IP.  
%Table~\ref{tab:ipvolumeavscore} to highlight the top-10 IPs.} 
%\label{Fig:results:ip_avscore_cdf}
%\end{figure}

%Figure~\ref{vt:ips:maliciousness} shows the distribution of number average number of positives per IP that correspond to malicious activities classes. While Table~\ref{tab:vt:ip:volume:avrank} contains the detail analysis of malicious files, urls, domains, and referrers that correspond to IPs in our dataset. We find that the average number of malicious URLs per IP is \red{XX $\pm$ STD} with average AV-rank equals \red{YY $\pm$ STD}. In Figure~\ref{vt:ip:urls}, we observe that \red{x\%} of the IPs have VT-rank at least 3. On a closer look, the figure suggests that IPs that correspond to Phishing have higher VT-rank i.e., more malicious than the IPs correspond to other classes of malicious activities.

%We find that the average number of malicious domain per IP is \red{XX $\pm$ STD} with average AV-rank equals \red{YY $\pm$ STD} .  In Figure~\ref{vt:ip:domains} (\ik{redo the domains per ip}), we observe that \red{x\%} of all IPs have AV-rank at least \red{y} while IPs that correspond to \red{Malware} class of malicious activities are more malicious in term of hosting malicious domains. 
%%
%On the hand, in Figure\ref{vt:ip:files} and Figure~\ref{vt:ip:referrers}, we observe that Phishing and Spammers IPs are more malicious, respectively, when compared to the rest of IPs that correspond to classes of malicious activities i.e., Malware, PUP, Exploits and PUP. 
%

%\ik{Edit the following paragraph once we have new results in Table~\ref{tab:ipvolumeavscore}.}

In Table~\ref{tab:ipvolumeavscore}, we show volume and AV-Score of the top 5 IP addresses in our dataset. We observe that \texttt{69.172.216.56} that hosted in AS7415 (Integral Ad Science, Canada)  is predominantly {\it specialized} in PUP (35.8K ) with AV-Score of 96\%. Similarly, \texttt{109.70.128.156}, is hosted in AS45037 (HispaWeb-Network, Spain), participated in 18.4K Mal-Activities that correspond to Malware and Exploits categories and has total AV-Score 46\%.
 
\begin{table}[ht!]
\centering
\scriptsize
%\Small
\vspace{-0.2cm}
\tabcolsep=0.04cm
\begin{tabular}{rr rrrrrrrrrrrrr}
\toprule
&  \multicolumn{2}{c}{\bf Malware} & \multicolumn{2}{c}{\bf Phishing}& \multicolumn{2}{c}{\bf Spam.}& \multicolumn{2}{c}{\bf Exploits}& \multicolumn{2}{c}{\bf PUP}& \multicolumn{2}{c}{\bf FS}& \multicolumn{2}{c}{\bf Total}\\
IP	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	&	Vol.	&	AVS.	\\
69.172.216.56	&		&		&	1	&	96\%	&		&		&		&		&	35.8K	&	96\%	&		&		&	35.8K	&	96\%	\\
109.70.128.156	&	17.4K	&	46\%	&		&		&		&		&	1.2K	&	46\%	&		&		&		&		&	18.6K	&	46\%	\\
61.160.210.226	&		&		&	18.5K	&	85\%	&		&		&		&		&		&		&		&		&	18.6K	&	85\%	\\
221.229.204.145	&		&		&	18.6K	&	85\%	&		&		&		&		&		&		&		&		&	18.6K	&	85\%	\\
59.45.79.75	&		&		&	16.4K	&	85\%	&		&		&		&		&		&		&		&		&	16.4K	&	85\%	\\
%54.235.91.69	&	13.1K	&	76\%	&		&		&		&		&	2.8K	&	76\%	&		&		&		&		&	15.8K	&	76\%	\\
%54.204.8.151	&	12.9K	&	76\%	&		&		&		&		&	2.7K	&	76\%	&		&		&		&		&	15.6K	&	76\%	\\
%62.76.103.211	&	8	&	13\%	&		&		&		&		&	1	&	13\%	&		&		&	13.3K	&	13\%	&	13.3K	&	13\%	\\
%107.22.195.95	&	10.9K	&	76\%	&	2	&	76\%	&		&		&	1.5K	&	76\%	&		&		&		&		&	12.4K	&	76\%	\\
%23.23.201.174	&	11K	&	76\%	&	6	&	76\%	&		&		&	1.4K	&	76\%	&		&		&		&		&	12.4K	&	76\%	\\
\bottomrule
\end{tabular}
\caption{\small Volume (Vol.) and AV-score (AVS.) of top-5 IPs.}% FS represents fraudulent services (a class of malicious activities) and country code, respectively. }
\vspace{-0.9cm}
\label{tab:ipvolumeavscore}
\end{table}

%As the volume (and AV-score) analysis of IPs do not reveal the participation in different classes of Mal-Activities, therefore, in the following subsections, we use our affinity and {\it specialization} and {\it affinity} metrics (see Section~\ref{sec:metrics}) to further analyze the IPs in our dataset. 
%
%\begin{figure*}[h]
%\centering
%%\subfigure[\small]{\includegraphics[width=1\columnwidth, height=0.4\columnwidth]{./plots/mplots/ips/malicious_urls_on_ips.pdf}}
%\subfloat[\small Malicious \textit{URLs} on IPs]{\includegraphics[width=0.25\textwidth,height=0.12\textwidth]{./plots/mplots/ips/detected_urls_samples_combined_attacks_mean.pdf}\label{vt:ip:urls}}
%\subfloat[\small Malicious \textit{Domains} on IPs (\red{redo it})]{\includegraphics[width=0.25\textwidth,height=0.12\textwidth]{./plots/mplots/domains/vt_positives_domains_combined_attacks_mean.pdf}\label{vt:ip:domains}}
%\subfloat[\small Malicious files on IPs]{\includegraphics[width=0.25\textwidth,height=0.12\textwidth]{./plots/mplots/ips/detected_download_samples_combined_attacks_mean.pdf}\label{vt:ip:files}}
%\subfloat[\small Malicious \textit{referrers} on IPs]{\includegraphics[width=0.25\textwidth,height=0.12\textwidth]{./plots/mplots/ips/detected_referer_samples_combined_attacks_mean.pdf}\label{vt:ip:referrers}}
%
%\hspace{-0.3cm}
%\caption{VT-Analysis: Distribution of malicious \textit{referrers} by IPs associated with different attack classes. \red{redo this figure, with: 1. all (labelled \& unlabelled), 2. all labelled, and 3. use max with STD mal positives.} } 
%\label{vt:ips:maliciousness}
%\end{figure*}
%%
%
%\begin{table}[h!]
%\centering
%\scriptsize
%\tabcolsep=0.040cm
%%\subfloat[Malicious Files on IPs]{\label{tab:tab1a}\scalebox{1.0}{
%\begin{tabular}{lcccccc}
%\toprule
%{\bf VT-Rank} & {\bf Malware}  	&	{\bf Phishing}  &	{\bf Spam.}  &	{\bf PUP} &	{\bf Exploits} &	{\bf FS}\\
%\midrule
%1	&	22\%&	18\%		&	19\%		&	36\%		&	21\%&	32\%		\\
%2	&	~9\% &	~6\%		&	~6\%		&	10\%		&	~7\%&	~9\%		\\
%3	&	~5\%&	~4\%    &   ~5\%		&	~5\%		&	~5\%&	~5\%		\\
%$\geq$4	&	64\%&	72\%	&	70\%		&	49\%		&	67\%	&	54\%	\\
%\bottomrule
%\end{tabular}
%\caption{Distribution of Malware positives of malicious files on IPs. }%`AV-rank'' means the number of VirusTotal's anti-virus tools that identified (Table \ref{tab:tab1a}) files and (Table \ref{tab:tab1b}) referrers of IPs as malicious. 
%%}
%\label{tab:tab1}
%\end{table}

%
%\begin{table}[h]
%\centering
%\scriptsize
%\tabcolsep=0.080cm
%\begin{tabular}{lcccccccc}
%\toprule
%         & \multicolumn{2}{c}{URLs} & \multicolumn{2}{c}{Domains} & \multicolumn{2}{c}{Files} & \multicolumn{2}{c}{Referrers} \\ \hline
%All      & 7701660 & 0.057 & 1318929 & 0.0416 & 807336 & 0.307 & 17645 & 0.346 \\
%Malware  & 4407627 & 0.061 & 878943  & 0.0431 & 370367 & 0.292 & 9341  & 0.361 \\
%Phishing & 2475829 & 0.060 & 388882  & 0.0454 & 340248 & 0.356 & 2439  & 0.227 \\
%PUP      & 291049  & 0.032 & 54758   & 0.0360 & 25820  & 0.220 & 990   & 0.152 \\
%FS       & 1632375 & 0.047 & 418943  & 0.0391 & 117194 & 0.271 & 1883  & 0.389 \\
%Exploits & 282992  & 0.054 & 82409   & 0.0429 & 39072  & 0.323 & 2439  & 0.227 \\
%Spam.    & 14954   & 0.058 & 2381    & 0.0467 & 1894   & 0.286 & 550   & 0.380 \\
%%All      & 176613 & 0.050 & \red{x} & \red{x} & 93570 & 0.201 & 2023 & 0.303 \\
%%Malware  & 93312  & 0.055 & \red{x} & \red{x} & 51434 & 0.187 & 1116 & 0.317 \\
%%Phishing & 36873  & 0.057 & \red{x} & \red{x} & 25828 & 0.208 & 237  & 0.217 \\
%%PUP      & 7175   & 0.027 & \red{x} & \red{x} & 2405  & 0.115 & 43   & 0.184 \\
%%FS       & 41364  & 0.039 & \red{x} & \red{x} & 17733 & 0.153 & 178  & 0.268 \\
%%Exploits & 7788   & 0.046 & \red{x} & \red{x} & 2690  & 0.212 & 227  & 0.292 \\
%%Spam.    & 532    & 0.045 & \red{x} & \red{x} & 131   & 0.243 & 25   & 0.449 \\
%\bottomrule
%\end{tabular}
%\caption{Malicious URLs, files, referrers, and domains that correspond to IPs in our dataset. Here Volume means the number of malicious URLs, files, referrers, or domains while AV-R. means average AV-Rank that correspond to the volume values. }
%\label{tab:vt:ip:volume:avrank}
%\end{table}

%
%\begin{table}[h!]
%\centering
%\scriptsize
%\tabcolsep=0.040cm
%\subfloat[Malicious Files on IPs]{\label{tab:tab1a}\scalebox{1.0}{
%\begin{tabular}{lcccccc}
%\toprule
%{\bf VT-Rank} & {\bf Malware}  	&	{\bf Phishing}  &	{\bf Spam.}  &	{\bf PUP} &	{\bf Exploits} &	{\bf FS}\\
%\midrule
%1	&	22\%&	18\%		&	19\%		&	36\%		&	21\%&	32\%		\\
%2	&	~9\% &	~6\%		&	~6\%		&	10\%		&	~7\%&	~9\%		\\
%3	&	~5\%&	~4\%    &   ~5\%		&	~5\%		&	~5\%&	~5\%		\\
%$\geq$4	&	64\%&	72\%	&	70\%		&	49\%		&	67\%	&	54\%	\\
%\bottomrule
%\end{tabular}
%}}\qquad
%\subfloat[Malicious Referrers of IPs]{\label{tab:tab1b}\scalebox{1.0}{
%\begin{tabular}{lcccccc}
%\toprule
%{\bf VT-Rank} & {\bf Malware}  	&	{\bf Phishing}  &	{\bf Spam.}  &	{\bf PUP} &	{\bf Exploits} &	{\bf FS}\\
%%{\bf \# Malware}  	&	{\bf Phishing}  &	{\bf Spammers}  &	{\bf PUP} &	{\bf Exploits} &	{\bf Fraudulent Services}\\
%\midrule
%1	&	~9\%&	21\%		&	~4\%		&	52\%		&	13\%&	~9\%		\\
%2	&	~4\% &	~7\%		&	~0\%		&	10\%		&	~7\%&	~3\%		\\
%3	&	~3\%&	~8\%    &   ~1\%		&	~6\%		&	~6\%&	~1\%		\\
%$\geq$4	&	84\%&	64\%	&	95\%		&	38\%		&	76\%	&	87\%	\\
%
%\bottomrule
%\end{tabular}
%}}
%\caption{Distribution of Malware positives of malicious files on IPs. `AV-rank'' means the number of VirusTotal's anti-virus tools that identified (Table \ref{tab:tab1a}) files and (Table \ref{tab:tab1b}) referrers of IPs as malicious. %\ik{@Ikram, VT number of malware positives per IP distribution for malicious files and URLs.}
%}
%\label{tab:tab1}
%\end{table}


%\textbf{Maliciousness of Domains:} Table~\red{IncludeTable}, shows the distribution of number of positives per domain in attack attack classes.  

%\textbf{Maliciousness of domains content categories:} Table~\red{IncludeTable}, we correlate the maliciousness with domains' content categories.


%\subsection{Domains Content Analysis} 
%\label{subsec:m_content_analysis}
%Using VT domains' content type in dataset, we map content type to domains in our dataset and highlights the distribution of content classes in attack classes. 
%\red{@Ikram/Ben: Include figure or table to show the distribution of domain content classes in each attack.} 

%\subsection{Hosts maliciousness analysis}

%\subsection{Affinity of IPs and Domains.}
\subsection{Affinity and Specialization of IPs}
\label{subsec:ip_specialization}
%In the previous section, we observe the Volume and maliciousness of IP addresses in our dataset. 
%Using our Affinity and Specialization metrics, detailed in Section~\ref{sec:metrics}, we measure IP addresses' contributions to six different classes of malicious activities (see Section~\ref{sec:mtypes}). 
The volume (and AV-score) analysis of IPs does not reveal the participation in different categories of Mal-Activities, therefore, we leverage our {\it affinity} and {\it specialization} metrics (see \S~\ref{sec:metrics}) to further analyze the IPs in our dataset. 
%Figure \ref{Fig:results:attk_prob_cdf:IP} shows the cumulative $P(n)$ (cf. Equation~\ref{eqn:attack_affinity}) of each the IP addresses in the six different classes of malicious activities. For the proportion of the IP addresses' contributions, we observe a trend between the attacks. IPs contributions to malicious activity class follow the order from least to the most for Malware and Spammers classes of malicious activities, respectively. %As we move from Figure \ref{Fig:results:ip_attk_prob_cdf} to \ref{Fig:results:asn_attk_prob_cdf} to \ref{Fig:results:cc_attk_prob_cdf}, we observe that the larger coverage of host on the ASN and CC level will each hold more of the occurrence distribution, as is expected.

%\begin{figure}[h]
%\centering
%%\subfloat[\small IPs]{
%\includegraphics[width=0.48\textwidth,height=0.17\textwidth]{./plots/eplots/ip_prob.pdf}\label{Fig:results:ip_attk_prob_cdf}
%%}
%%\subfloat[\small ASNs]{\includegraphics[width=0.33\textwidth]{./plots/eplots/asn_prob.pdf}\label{Fig:results:asn_attk_prob_cdf}}
%%\subfloat[\small CCs]{\includegraphics[width=0.33\textwidth]{./plots/eplots/cc_prob.pdf}\label{Fig:results:cc_attk_prob_cdf}}
%\caption{Affinity of IPs and \ik{Domains, TODO}: CDF of the Probability that an IP and Domain \ik{todo} is selected from the set of contributing hosts of a particular attack class. \ik{this does not add much. delete it}}% \ben{This plot shows the probability of selecting a host from the set of hosts within a particular type of malicious activity (when considering reports).}} 
%\label{Fig:results:attk_prob_cdf:IP}
%\end{figure}

%Table \ref{tab:ip_affinity_purity} contains columns for the affinity of malicious activity classes. From a high level, between the teirs of infrastructure we can observe the decreasing entropies as more reports begin to aggregate under a smaller number of labels (asn, cc), this aggregation and the decrease in the value of entropy indicates the more significant contribution by a few particular labels, opposed to the labels being even contributors to the type of malicious activities. 
%This Shannon Diversity index (entropy) conclusion is backed up by the previously mentioned Figure \ref{Fig:results:attk_prob_cdf:IP}, as we observe the gradient of the CDF and hence the distribution of labels within the lower probabilities decrease. In case there was no emergence of a significant contributing label the shape of the curve between a,b,c would remain the same but move towards the right to the lower probabilities.


%Table~\ref{tab:ip_affinity_purity}, we analyze the differences between the types of malicious activities in terms of Affinity of IPs (see Section~\ref{subsec:entropymetrics}). % We consider the IP column of Attack %Affinity within Table \ref{tab:ip_affinity_purity}, 

{\bf Specialization and Affinity.}  %Table~\ref{tab:ip_affinity_purity} shows the results of our analysis. 
Figure \ref{Fig:results:attk_cdf}, shows that there is a significant portion of IPs (80\%) that participate in only category of Mal-Activities. While measuring the IPs' affinity, we observe that the PUP has the highest affinity (0.871) while Exploits has the least (0.794). Phishing, Fraudulent services, Malware have second, third, and fourth highest affinities (0.801, 0.815, and 0.834 respectively) while Spammers category has the second-highest (0.847). When compared to other categories, interestingly, the smaller affinity of Exploits--at least 0.7\% smaller than the all other category--suggesting that a subset of IP addresses contributes most of the Exploits. On the other hand, IPs that corresponding to the PUP are {\it equally} contributing to this category of Mal-Activities. 

%In Section~\ref{subsec:gdistribution} and Section~\ref{subsec:infrastructure}, we shall further analyze the participation of countries and ASes, respectively, in these six classes of malicious activities. 

%to the PUP class of malicious activities are ``originated'' from specific group of IP addresses. 

%Moreover, we shall see in Section [\red{x}] [\red{x}] and 0.22 less within CCs, this decrease would indicated that the proportion of Unwanted programs is much more concentrated on a few IPs within it's reported set of IPs, and moving across the tiers we can consistently observe this trend, indicating that Unwanted programs are much more concentrated among a few ASes and Countries, as compared to their counterparts.  %I also bring to light the usefulness of Entropy as a metric that a basic CDF of probability excludes, from Figure \ref{Fig:results:attk_prob_cdf:IP} 
%Moreover, in Figure~\ref{Fig:results:attk_prob_cdf:IP}, we observe that Spammers is consistently the rightmost line.  but this is inpart due to the lower of initial reports within this type of malicious activity (i.e. x axis is not normalized between attack types, more empirical comparison), The Shannon Diversity index however allows an 'fair' comparison between the probability distributions.

%\begin{table}[h!]
%\centering
%\scriptsize
%\begin{tabular}{ rrrrrrrr }
%\toprule
%\toprule
%{\bf Metric} & {\bf PUP} & {\bf FS} & { \bf Malware}&{\bf Exploits}&{\bf Phishing} &{\bf Spammers}&{\bf Total}\\
%\midrule
%Affinity &  0.871 & 0.815 & 0.834& 0.794& 0.801& 0.847& 0.820\\
%%Speci. &0.0352	&     0.133	& 	0.592&	0.0273& 	0.102 	&   0.00196&	0.109\\ % Ben says this row is useless. Indeed isn't specialization, its just the p(n) used in measuring specialization.
%\bottomrule
%\end{tabular}
%\caption{Affinity of IPs in our dataset.}%The IPs specialization and malicious activities class affinity.  Here UL represent ``unlabelled'' malicious activities (see. Table~\ref{tab:dataset}) in our dataset. \ik{As we can mention these numbers in text, perhaps, we should kick this table out. Suggestions?} \red{Remove 'UL' and add 'LB'--total labelled malicious activities.}
%%}
%\label{tab:ip_affinity_purity}
%%\vspace{-1.0cm}
%\vspace{-0.2cm}
%\end{table}

%\begin{table}[h]
%\centering
%\begin{tabular}{ rc c }
%\toprule
%       		 &  \multicolumn{2}{c}{IPs} \\
%\toprule
%Mal. Activity Class & Affinity & Specialization\\
%\midrule
%Unwanted Programs 	& 0.594   	&     	0.0352 \\
%Fraudulent Services  	& 0.804   	&     0.133 \\
%Malware            		& 0.778    	& 	0.592 	\\
%Exploits           			& 0.799   	&	0.0273 	\\
%Phishing         			& 0.812	& 	0.102 	\\
%Spammers			& 0.770    	&     	0.00196 	\\
%Unlabelled			& 0.782	&	0.109	\\
%\bottomrule
%\end{tabular}
%\caption{The IPs affinity to malicious activity class. \ben{There is pending work Regarding the normalization of the Host Specialization values, Attack affinity is fine.}}
%\label{tab:ip_affinity_purity}
%\vspace{-1.4cm}
%\end{table}


%\subsection{Specialization of IPs and Domains} 
%\subsection{Specialization of IPs} 
%\label{subsec:ip_specialization}

%{\bf Specialization.}  %To measure the distribution of IPs across classes of malicious activities, we rely on our Specialization metric (see Section~\ref{sec:metrics}). 
%
%Figure \ref{Fig:results:attk_cdf}, shows that there is a significant portion of IPs (80\%) that participate in only category of Mal-Activities. However, when we analyze malicious activities at ASN and country level, we observe a more uniform distribution of the attack classes within the hosts. For instance, the CDF curves shifting the bulk of their proportion towards the higher values of entropy (more disorder = more spread amongst the classes).  

%[From This plot we can observe with the 0 entropy values, the proportion of the various tiers, and their tendency to not be diversely spread amongst the different types of malicious activity, Additionally from the reach into the x axis, we can observe as you aggregate into the higher tiers of infrastructure, the Specialization to a par- ticular type of malicious activity decreases, as indicated by the higher value of entropy (a more even distribution of a entities oc- currences over the types of activities.) ?BZ]

%We use ASN-rank and AS-classification dataset to further analyze the participation of ASes in different malicious activities. %\ik{@Ikram/Ben: TODO: Produce and discuss results.}

%can further enrich this line of analysis by considering the different types of Hosts available e.g. hosting/transit/commercial/private, etc. However in order to do so we will need additional datasources as inputs.


\begin{figure}[ht!]
\vspace{-0.4cm}
\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/Combined-Attk-Entropy_CDF.pdf}
\includegraphics[width=1\columnwidth]{markered_plots/Combined-Attk-Entropy_CDF-crop.pdf}
\vspace{-0.8cm}
\caption{\small IPs, ASes, Cities, and Countries Specialization}%: CDF of Shannon Entropy of Hosts.}% based on a Specific Entities spread/specialization to a specific type of malicious activity. }
\vspace{-0.2cm}
\label{Fig:results:attk_cdf}
\vspace{-0.4cm}
\end{figure}


==> files/metrics.tex <==
%In this section, we briefly explain the metrics we used to analyze the malicious activities in collected dataset. 

\subsection{Metrics in use}

To better understand how malicious activities are distributed amongst IPs, ASes and Geolocations, we first introduce two diversity (or a homogeneity) metrics named \emph{Affinity} and \emph{Specialization} adopting \textit{Shannon entropy}. Then, we introduce \emph{AV-Score} that quantifies the prevalence of malicious activities among many Anti-Virus scanners and databases. These three metrics are used throughout the paper for retrospective spatiotemporal analysis of mal-activity distribution.

{\bf Affinity.} To measure the spread of a given class of malicious activity (cf. \S~\ref{sec:mtypes}) across reported malicious Hosts, we define \emph{Affinity} as normalized Entropy per malicious activity $a$ as $A(a) = (-\sum_{\forall h} P(h) \log_2{P(h)})/\log_2 k$ where;
\begin{equation} \label{eqn:attack_affinity}
P(h) = \frac{\# \, \text{of reports from host $h$ with activity $a$}}{\text{Total} \, \# \, \text{of reports}}
\end{equation}
In this regard, $A(a)=1$ represents that reports of malicious activity $a$ are evenly distributed among all hosts and conversely $A(a)=0$ represents that all reports are concentrated on a single host. 

{\bf Specialization.} The distribution of hosts across classes of malicious activities is defined as normalized Entropy per host $h$ as  $S(h) = (-\sum_{\forall a} P(h) \log_2{P(h)})/\log_2 k$ where the probability $P(h)$ is defined as in Equation ~\ref{eqn:attack_affinity}. 
%\begin{equation} \label{eqn:host_specialization}
%P(a) = \frac{\# \, \text{of reports from host $h$ with activity $a$}}{\text{Total} \, \# \, \text{of reports}}
%\end{equation}
Strong specialization of hosting one particular malicious activity class is represented by higher $S(h)$ value for a given host $h$.

{\bf AV-Score.}
It is imperative to rely on multiple AV scanners and databases to filter malicious activities as they often attempt to circumvent certain AV tools and also to reduce false positives~\cite{6234407}. Furthermore, having noted by multiple AV scanners is an indication of prevalence of the malicious activity. We define \emph{AV-Score} to quantify the maliciousness of an activitiy such that $\text{AV-Score}(h) = \frac{\sum_{i=1}^{N} \mathcal{P}_i}{N}$ where $\mathcal{P}_i$ equals $1$ if an AV tool, $i$, flags a given host $h$ as malicious, otherwise $\mathcal{P}_i$ equals $0$. $N$ is the total number of available AV-tools\footnote{As of May 15$^{th}$,  2017, VirusTotal used 68 different AV-tools to check malicious activities.} used by VirusTotal to determine malicious activities of a host.

%\begin{equation}
%    \text{AV-Score}(h) = \frac{\sum_{i=1}^{N} \mathcal{P}_i}{N} \; \text{where}  \; \mathcal{P}_i =
%    \begin{cases}
%    1 & \text{if  $i$ flags $h$ as malicious}\\
%    0 & \text{otherwise}
%\end{cases}
%%\]
%\end{equation}



%\subsection{Affinity and Specialization}
%\label{subsec:entropymetrics}
%%\ik{NOTE: We need to define Hosts as ``general term'' to refer to domain/IP, ASN, and country. In this subsection, we have to restrict ourselves to domain/IP only. We will discuss the `attack affinity' and `host (country and asn) specialization' in subsection~\ref{subsec:gdistribution} and subsection{subsec:infrastructure}. }
%
%To better understand how malicious activities are distributed amongst IPs, ASes and geolocations, we first introduce a diversity (or a homogeneity) metric. We adopt \textit{Shannon entropy} , $H(X)$ (see Equation \ref{eqn:shannon}),  as it is easy to understand and compute and can be adapted to many contexts (e.g., time series data). Specifically, we use the normalized version of this equation (see Equation \ref{eqn:norm_shannon}) that outputs a value between zero and one.   
%
%\begin{equation}
%\label{eqn:shannon}
%H(X) = -\sum_{n=1}^{k} P(n) \log_2{P(n)} 
%\end{equation}
%
%\begin{equation}
%\label{eqn:norm_shannon}
%H_{n}(X) = \frac{H(X)}{\log_2{k}}
%\end{equation}
%
%To briefly elaborate this metric, let us compute normalized Shannon entropy, $H_{n}$, for three different scenarios. First, we consider a single malicious class with three participants (e.g., IPs or country) contributing $\frac{1}{16}, \frac{5}{16}, \frac{10}{16}$ each respectively. The resulting Shannon entropy would then be $\Big(\frac{1}{16} \log_2{\frac{1}{16}}\Big) - \Big(\frac{5}{16} \log_2{\frac{5}{16}}\Big) - \Big(\frac{10}{16} \log_2{\frac{10}{16}}\Big) = 1.1982$ therefore $ H_{n}(X) = \frac{H(X)}{\log_2{3}} = 0.756$. Second, consider the same scenario but with participants contributing equally (i.e., $\frac{1}{3}$). This will lead to $H_{n}(X)=1$. Finally, suppose that a single entity is at the origin of a malicious class (i.e., $1$) then $H_{n}(X)$ would be equal to zero.
%
%From these examples we can observe that the normalized Shannon entropy is equal to zero if the probability distribution is condensed in a single point and one if the probability is evenly distributed among all participants. Numbers in between depict shift to either of these extremes.
%%
%%\beriw{Here you define Shannon entropy + examples and then??? Nothing happens!!!! We moved to an entirely new section that has nothing to do with this paragraph. The link to equation 2 is not clear as you are computing occurrences. You are also referring to entropy while I see none. The next two paragraphs are unparsable for me while I can see what was your goal I was not able to get anything out of the text so please REFORMULATE. }
%%\beriw{ START UNPARSABLE }
%%
%%\ben{This section serves to introduce the Shannon Index (Shannon Entropy) as a means of measuring disorder/diversity within different combinations of parameters within our dataset, I have provided the general definition and examples to provide context for what follow in the next section and later on in the Temporal section, i.e. what does 1 or 0 similarity mean?}
%%
%We use the aforementioned Shannon entropy to investigate the Host's (i.e., domain, IP, ASN, or country) participation in different classes of malicious as defined in Section~\ref{sec:mtypes}. In essence, we use $P$ (see Equation~\ref{eqn:shannon}) to define two metrics: {\it affinity} and {\it specialization}.
%%\begin{enumerate}
%%\item The \textit{Affinity} of reports over contributing Hosts, within an attack class
%%\item The \textit{Specialization} to a specific Attack Class, within an attack class.
%%\end{enumerate}
%%
%%\subsubsection{Attack Affinity}
%
%{\bf Affinity.} To measure the spread of a given class of malicious activities across participating Hosts, we define affinity. Formally, it is the probability of a Host that correspond to a class of malicious activity (see Section~\ref{sec:mtypes}):
%
%\begin{equation} \label{eqn:attack_affinity}
%P(n) = \frac{K(n)}{\sum_{n=1}^{m} K(n)} , K \in \text{malicious activities' class (cf. \S~\ref{sec:mtypes})},
%\end{equation}
%where $m$ and $K(n)$ are the total number of hosts in malicious activities' class and frequency of a host, $n$, respectively. %and $K(n)$ is the number of occurrences of a host, $n$.
%%
%The high value of entropy (i.e., $H_{n}(X)$) on the scale from $0.0$ to $1.0$, measured with $P(n)$ in Equation~\ref{eqn:attack_affinity}, will suggest that the malicious activity are more evenly distributed across the contributing hosts. Conversely, it is true for low value of $H_{n}(X)$. 
%
%%From this definition we can examine the behavior of the Attack Class in regards to how the Attack as an entity utilizes the Hosts i.e., wether it aims to divide it's attack vectors, without a concentration on a few key Hosts, or to have a homogeneous approach across it's hosts. For this metric we have taken the subsets of the hosts for a particular attack in the entropy analysis as there is not a even distribution of hosts among the attacks, which will consequently skew the resulting comparison.
%
% 
%%\subsubsection{Host Specialization}
%{\bf Specialization. } %\ik{We need a better term e.g., Uniquenss.} 
%It measures the distribution of host across classes of malicious activities (cf. Section~\ref{sec:mtypes}) and is defined as: 
%%It is the frequency distribution of the occurrences over the attack classes for specific Host. 
%
%\begin{equation} \label{eqn:host_specialization}
%P_{j}(n) = \frac{K(n)}{\sum_{n=1}^{l} K(n)} , K \in \text{Host $j$},
%\end{equation}
%
%where $l$ is the total number of classes of malicious activities, and $K(n)$ is the number of occurrences of a give malicious activity class for a particular Host $j$. In other words, it determines if a Host is involved in a particular class of malicious activities or indiscriminately in more than one class of malicious activities. Thus a high value of entropy (i.e., $H_{n}(X)$), would suggest a high volume of malicious activities of given host that are evenly distributed across the classes of malicious activities.  Conversely, it is true for low value of $H_{n}(X)$. 
%
%%We perform this metric on subsets of Hosts belonging to the different Attack classes to obtain a measure of the Host Specialization for a particular attack type, from this metric it can be determined if a particular attack class's hosts are more or less specialized to the attack class in question or the hosts contribute to all attacks indiscriminately.
%\subsection{VirusTotal Rank}
%\label{sec:avrank}
%Software component that participate in malicious activities may circumvent a specific AV tool~\cite{6234407} Thus it is imperative to rely upon multiple AV scanners and datasets to effectively determine the degree of malicious of Hosts in our dataset.  Given that a single scanning tool may produce false positives~\cite{6234407}, we rely on the ``AV-Rank'' metric~\cite{Ikram:vpn} \ik{AV-rank and AV-score is interchangeably used throughout the paper. Use either AV-Rank or AV-Score.} (i.e., the number of affiliated AV tools that identified any malware activity) to reason about the maliciousness of an app. Formally, we define AV-Rank as follow:
%
%\begin{equation}
%%\[
%   AV-Rank(x) = 
%\begin{cases}
%    \frac{\sum_{i=1}^{N} \mathcal{P}_x^i}{N},& \text{if  $i$ flag $x$ as malicious}\\
%    0,              & \text{otherwise,}
%\end{cases}
%%\]
%\end{equation}
%where $\mathcal{P}_x^i$ equals $1$ if an AV tool, $i$, flags a given Host $x$ as malicious, otherwise $\mathcal{P}_x^i$ equals $0$. Here $N$ is the total number of AV tools\footnote{As of May 15$^{th}$,  2017, VirusTotal used 68 different AV-tools to check malicious activities associated with Hosts.} used by VirusTotal to determine malicious activities of a Host. 
%A high value of AV-Rank, on the scale from $0\%$ to $100\%$, will determine that a particular Host is highly malicious. While AV-Rank equals $0\%$ will suggest that the Host is safe and neither of the AV-tools have ever detected malicious activities that correspond to the Host.
%
%%\ik{remove the denominator $N$ if we are use the 'number of positives' instead of 'fraction of number of positives'. Run consistency check throughout the paper.}


==> files/relative_geo_asn_lvl_anlaysis.tex <==
The analyses in the previous section may have overlooked the countries, cities, and ASes with relatively smaller number of allocated IPs. In this section, we aim to analyze niche geolocations and ASes, in our dataset, that have relatively smaller allocated IP addresses. To do this, we use CIPB dataset~\cite{cipb} and AS-Rank dataset~\cite{as_rank} to garner the total number of allocated IPs per geolocation and AS, respectively. Measuring the ratio of number of malicious IPs to the IP block per country (resp. AS), we investigate the relative analysis of geolocations (resp. ASes).  This ratio allows us to avoid the biases due to the country (resp. AS) connectivity and size.  To measure the average AV-Score of Mal-Activities that originate from a geolocation, we leverage on VirusTotal dataset to measure the AV-Score of IPs that are geolocated in a country. Similarly, we measure the AV-Score of IPs correspond to Mal-Activities that are originated from an AS. 

%{\bf Relative malicious activities per geolocation:} 
\subsection{Country-Level Analysis} We show the CDFs of number of Mal-Activities per country in Figure \ref{fig:country_malicious_proportion}. We notice that Malware class of Mal-Activities (red line) follows similar trend as that of all Mal-Activities (black line). This suggests relatively high proportions of IPs per geolocation contributes to Malware class of Mal-Activities. Overall, the ratio of number of malicious IPs to the total number of IPs is low, however, the long-tail of the distributions (the top left) reveal geolocations with relatively high proportion of IPs participate in Mal-Activities. In Table \ref{tab:malicious_top10:proportion}, we list the top 5 geolocations that correspond to the tail (top left corner) of the distributions. Although, in Section~\ref{subsec:gdistribution} we observed that these geolocations where less aggressive in terms of volume of Mal-Activities, however, they have relatively high proportion of IPs participating in Mal-Activities according to our ratio. 


\begin{figure}[ht!]
\centering
\subfloat[\small Countries]{\includegraphics[width=0.24\textwidth]{new_plots/cc_attack_block_proportion.pdf}\label{fig:country_malicious_proportion}}
%\subfloat[\small Cities]{\includegraphics[width=0.33\textwidth]{new_plots/city_attack_block_proportion.pdf}\label{fig:city_malicious_proportion}}
\subfloat[\small ASes]{\includegraphics[width=0.24\textwidth]{new_plots/asn_attack_block_proportion.pdf}\label{fig:asn_malicious_proportion}}
\vspace{-0.45cm}
\caption{\small The proportion of IPs in a country (resp. AS) involved in Mal-Activities.}%to total number of allocated IPs per country (resp. AS). } 
\vspace{-0.6cm}
\label{fig:relativeanalysis}
\end{figure}


\begin{table}[h!]
\centering
\scriptsize
%\small
\tabcolsep=0.080cm
%\resizebox{0.69\textwidth}{!}{\begin{minipage}{\textwidth}
\subfloat[Geolocations]{\label{tab:country_malicious_top10:prop}\scalebox{0.69}{
\begin{tabular}{ r r r c r r r}
\toprule
% &    {\bf Mal.}      &  {\bf Total}   &  & &\\
{\bf CC}              &    {\bf Mal. IPs}      &  {\bf Tota IPs}   &  {\bf Ratio} & {\bf Vol.} & {\bf AVS.} \\
\midrule
NA	&	7615	&	463.5K	&	1.64		&	63K&	52\%	\\
VG	&	1394	&	135K	&	1.03	&	206K&	94\%		\\
AI	&	91	&	10.3K	&	0.89	&	222&	9\%		\\
LT	&	4690	&	2.7M	&	0.17	&	37K&	54\%		\\
BZ	&	302	&	178.5K	&	0.17		&	2K&	36\%	\\
%LU	&	1961	&	1.46M	&	0.13	&	13.4&	45\%		\\
%UA	&	12576	&	12.7M	&	0.10	&	26K&	57\%		\\
%VN	&	15220	&	15,9M	&	0.10	&	241K&	50\%		\\
%LR	&	81	&	103.2K	&	0.08	&	159&	49\%		\\
%MD	&	997	&	1.36M	&	0.07	&	14K&	61\%		\\
\bottomrule
\end{tabular}
}} 
%\quad
%\subfloat[Cities]{\label{tab:city_malicious_top10}\scalebox{1.0}{
%\begin{tabular}{rr  r r  c r r}
%\toprule
% & & {\bf Mal.} & {\bf Total} & &  & \\
%{\bf City} & {\bf CC} &{\bf IPs} & {\bf IPs} & {\bf Ratio} & {\bf Vol.} & {\bf AVS.}\\ %& {\bf CC} 
%\midrule
%Ursa	&	MX	&	117	&	1488	&	7.86	&	3.2K	&	90\%	\\
%Kentwood	&	US	&	164	&	3182	&	5.15	&	907	&	67\%	\\
%Baruun-Urt	&	MN	&	10	&	255	&	3.92	&	25	&	63\%	\\
%Rozendaal	&	NL	&	40	&	1272	&	3.14	&	436	&	47\%	\\
%Boesingheliede	&	NL	&	29	&	1011	&	2.87	&	108	&	52\%	\\
%%Wyandotte	&	US	&	539	&	26398	&	2.04	&	372K	&	93\%	\\
%%Ogmore-by-Sea	&	GB	&	5	&	254	&	1.97	&	17	&	61\%	\\
%%Nusttal	&	US	&	24	&	1276	&	1.88	&	291	&	39\%	\\
%%Ligne	&	FR	&	151	&	9950	&	1.52	&	1531	&	65\%	\\
%%Budva	&	ME	&	35	&	2326	&	1.5	&	113	&	83\%	\\
%\bottomrule
%\end{tabular}
%}}\qquad
%\resizebox{0.5\textwidth}{!}{\begin{minipage}{\textwidth}
\subfloat[ASes]{\label{tab:asn_malicious_top10:prop}\scalebox{0.69}{
\begin{tabular}{r r r r r  r r r r}
\toprule
% & & &&   &{\bf Mal.} & {\bf Total} &  & & \\
{\bf AS} &{\bf Org.}&{\bf AS-R}& {\bf AS-T} &  {\bf Mal. IPs} & {\bf Total IPs} & {\bf Ratio} & {\bf Vol.} & {\bf AVS.}\\
\midrule
31624	&	VFMNL, NL	&	23423	&	Co	&	2471	&	4,352	&	56.8	&	12.3K	&	63\%	\\
44901	&	BelCloud, BG	&	41638	&	En	&	114	&	256	&	44.5	&	1.2K	&	74\%	\\
54761	&	Sambreel Serv. LLC., US	&	18401	&	En	&	425	&	1,280	&	33.2	&	1.5K	&	66\%	\\
133618	&	Trellian Pty. Ltd, AU	&	29389	&	Co	&	277	&	1,024	&	27.1	&	36.2K	&	83\%	\\
61969	&	TeamInternet,  DE	&	36809	&	Co	&	235	&	1,024	&	22.9	&	84.7K	&	92\%	\\
%47583	&	HOSTINGER	&	LT	&	9091	&	Co	&	3651	&	18,432	&	19.8	&	29.3K	&	55\%	\\
%22612	&	NAMECHEAP-NET	&	US	&	8649	&	Co	&	3092	&	15,872	&	19.5	&	42.8K	&	69\%	\\
%51468	&	ONECOM	&	DK	&	6884	&	Co	&	849	&	5,120	&	16.6	&	6.1K	&	61\%	\\
%56464	&	VIBRANT	&	GB	&	41638	&	En	&	38	&	256	&	14.8	&	136	&	7\%	\\
%47846	&	SEDO-AS	&	DE	&	20859	&	Co	&	164	&	1,280	&	12.8	&	14.2K	&	83\%	\\
\bottomrule
\end{tabular}
}}%\end{minipage}}
\vspace{-0.4cm}
\caption{\small Top 5 countries (\ref{tab:country_malicious_top10:prop}) and ASes (\ref{tab:asn_malicious_top10:prop}) with proportion of IPs involved in Mal-Activities.}%}the ratio of number of malicious IP to the total  number of allocated IPs per country and per AS respectively.}% In Subfigure (\ref{tab:asn_malicious_top10}), we obtain AS-rank (AS-R) and AS-type (AS-T) from Caida's AS-Rank~\cite{as_rank} datasets.  Whereas `co' stands for Content (hosing and distribution systems) and `en' represents Enterprise (university, companies, and end-user networks). }%Figure~\ref{fig:country_malicious_proportion} details the overall distribution of the ratio.}
\label{tab:malicious_top10:proportion}
\vspace{-0.8cm}
\end{table}
%Content (hosing and distribution systems), and Enterprise (university, companies, and end-user networks)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\bf Relative malicious activities per city: } %\ik{Due to missing city-level dataset, we did not perform city-level temporal analysis, as we do in case of IPs/ASes/Geolocations, I tend to cut this out from the paper. Thoughts?} 
%\subsection{City-Level Analysis}
%Similarly, we analyze the ratio of number IP addresses that correspond to Mal-Activities to the total number of IP addresses geolocated in a given city.  Figure \ref{fig:city_malicious_proportion} shows the CDF of this ratio. We analyzed the long-tail of the distribution for the city with relative high ratio of number IPs correspond to Mal-Activities to the total number of IPs. In Table \ref{tab:city_malicious_top10}, we list the top 10 cities within this plot. We observe that, overall, according the number occurrences of Mal-Activities, these cities are less aggressive in term of volume of Mal-Activities, however, when compared to the malicious IP ratio per geo-location, they have the highest number of malicious IPs to the total number IPs ratio. %\ik{Can we trace and refer reports if certain offenders originate from the listed cities by searching online blogs/tech-reports?}



%{\bf Relative malicious activities per AS:} 
\subsection{AS-Level Analysis} 
%We further analyze the proportion of malicious of IPs per AS by measuring the number of malicious IPs to the total number of IPs in an AS. We obtain the total number of IPs per AS from Caida' AS-rank dataset~\cite{as_rank}. 

Figure~\ref{fig:asn_malicious_proportion} show the results of our analysis.  Once again, the trend--with Malware class of malicious activities have the highest ratio while the Spammers have the least--is similar to the ones we observed in the aforementioned section. However, when compared to the relative malicious ratio at city- and geolocation-level, we observed that the distribution of ratios of all Mal-Activities (and their classes such as Malware and Phishing) are skewed more to the right, suggesting higher AV-Score of a subset of ASes. Table~\ref{tab:asn_malicious_top10} lists the top-10 ASes with high ratio of malicious IPs to the total number of IPs per AS. We observe that AS31624, VFMNL-AS located in the Netherlands,  has 44\% of IPs that participated in 12.3K Mal-Activities that correspond to five categoris: Malware, Spams, Phishing, Exploits, and Fraudulent Services. We notice that on 63\% of AV tools flagged these Mal-Activities as malicious. AS49087 (PodCem, UA) is the second and AS45020 (VanBT, HU) is the third in the list with 29\% and 25\% of IPs, respectively, participate in Mal-Activities.%\ik{search and reference if there is reported malicious activities in these ASNs}.





==> files/temp.tex <==
A malicious activity (or mal-activity) is when one Internet device inflicts harm or damage to another device. A mal-activity may have different objectives such as phishing for user-credentials, scanning for security vulnerabilities, or acting as a simple drop point for malicious payloads. Despite concerted efforts by researchers and the industry, instances of mal-activity still persist. Many studies attempt to shed light on the reasons behind persistence of mal-activities. However, these are either short-term studies or use datasets that are not publicly available. The result is a lack of historical (public) knowledge of mal-activities which would better inform investigators about their behavior, and help modify detection and prevention strategies accordingly. 

This paper presents a methodology for the collection and longitudinal measurement of behaviors in reported mal-activities on the Internet from January 2007 to June 2017. A total of 51.6M mal-activity reports are collected involving 662K unique IP addresses worldwide. Our method leverages the Internet Wayback Machine, antivirus (AV) tool reports, and several additional datasets to enrich the data with historical meta-information including geolocation (countries) and infrastructure (autonomous system (AS) numbers). We categorize the collected mal-activities into six classes: malware, phishing, fraudulent services, spammers, exploits, and potentially unwanted programs (PUPs). 

Our findings reveal that a high number of hosts (IP addresses, ASes and countries) are highly specialized to a single class of mal-activity. Our results agree with the expectation that there is a larger contribution to mal-activities by countries with established IT infrastructure, and a preference of malicious actors to leverage cloud service providers to perform mal-activities.

An overview of the mal-activities over the ten year span reveals the rise of the mal-activity phishing, equaling malware in terms of volume of activities. Through modeling of the temporal behavior of mal-activities at both the AS and country level, we identify the most {\it frequent} and {\it active} participants. The previously undiscovered participants appear on a timescale which is not feasibly detectable through a short-term study. By proposing a number of techniques and metrics to summarize trends within longitudinal datasets, we obtain insights into the spatial and temporal behaviors of mal-activities, whilst providing new tools of analysis that can be extended beyond our dataset. We plan to release our unique ten-year long dataset to the research community for further analysis.  




\begin{table}[ht!]
\centering
%\vspace{-0.2cm}
\scriptsize
%\small
\tabcolsep=0.040cm
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ r c | c l c | c c  }
\toprule
{\bf IP}	&	{\bf Severity}	&	{\bf ASN}	& {\bf Org.} &	{\bf Severity}	&	{\bf CC}	&	{\bf Severity} \\
\midrule
54.230.14.36	&	34024	&	6762	&	SEABONE-NET, IT	&	2113	&	US	&	76493	\\
54.192.117.7	&	33976	&	35994	&	AKAMAI-AS, US	&	1659	&	CN	&	338	\\
54.192.146.82	&	33921	&	53684	&	FLASHPOINT-SC-AS-1, US	&	1607	&	DE	&	204	\\
54.192.195.247	&	33920	&	134418	&	CHINATELECOM, CN	&	1558	&	FR	&	109	\\
54.192.145.112	&	33920	&	16509	&	AMAZON-02	&	1523	&	BO	&	70	\\
\bottomrule
\end{tabular}
}
%\vspace{-0.25cm}
\caption{\small Severity analysis of Top 5 IPs, ASes, and Countries.}
\label{tab:severity:analysis}
%\vspace{-0.3cm}
\end{table}

==> files/temporal_analysis-old.tex <==
%In the previous sections, we provided a bottom up analysis of malicious activities starting from an IP based analysis and moving forward to characterize the diversity and the specialization of Hosts and geolocations. 


%We know focus on a different aspect: the \textit{temporal} evolution and behavior of malicious activities.  

The main contribution of this paper is the temporal Analysis of the mal-activity reporting behavior. We start by observing the volume of each class of reported malicious activity in our dataset over time. Obviously the seed dataset \textit{Blacklist-07-17} corresponds to different time ranges and so as mentioned earlier, might be biased towards specific periods of time where a particular mal-activity class would be more aggressively reported than others. However our use of Virus Total reports spanning the whole 2007-2018 period is intended to overcome that limitation as we believe the extensive number of Anti Virus products and their corresponding reports would be providing a comprehensive scan of the whole reporting period.   


\subsection{Evolution of the reporting of Malicious Activities} 

%Contrary to MDL~\footnote{http://www.malwaredomainlist.com}, several blacklists do not timestamp malware reports. In order study the evolution of malware in a given malware list (resp. all malware lists), we plan to use VirusTotal to obtain the first reported dates of malware. 
%\ik{@Beri and @ Kanchana: could you pass over this section and refine it a bit?}
%We begin our temporal analysis of analyzing the Volume or number of malicious activities over time i.e. evolution. We use the reported time-stamps of malicious activities within our dataset and measure the volume of malicious activities per day.  Figure~\ref{fig:evolution} shows the evolution of the different types of malicious activities. 
%
%\ik{Explain at least two key insights from the figures. Are attack classes increasing or decreasing over time? } 
%
%\ik{Use historical dataset from domz.com to reveal the types of URLs/Domains and, likewise, plot the evolution of type of urls/domains.} 

%Recall from Section~\ref{subsec:datasummary} that our historical data spans a 10 years period allowing us to shed light on how different malicious activities flourished over that time. 

Figure~\ref{fig:evolution} shows the evolution of classes of mal-activity in the \textit{VTBlacklist} data. Overall, malicious activities reporting has constantly increased over the last decade (black line) with an interesting spike around late 2008 beginning of 2009 driven by a significant increase in Fraudulent services and Exploits. 

Indeed, ExploitKits,  web based softwares that automatically exploit user's browser to install malwares, were first introduced in 2006 with Mpack and saw an exponential growth in the next 4 years\footnote{\url{https://blog.malwarebytes.com/cybercrime/2013/02/tools-of-the-trade-exploit-kits/}}. Malwares, and despite all collective efforts to thwart them, continue to increase in volume as well as in damage with new variants like ransamwares infecting hundred of thousands of computers.   

%\beri{We should reintroduce the plot with data availability over time. This will help in explaining the flat lines that we see in the plot. @Ik: add more findings here if you have}

\begin{figure}[ht!]
\centering
\subfloat[Coverage]{\label{fig:source_coverage}
\includegraphics[width=0.49\columnwidth,height=0.30\columnwidth,keepaspectratio]{plots/sources_coverage.pdf}}
\subfloat[Evolution ]{\label{fig:data_evolution} \includegraphics[width=0.49\columnwidth,height=0.30\columnwidth,keepaspectratio]{new_plots/all_attacks_evolution.pdf}}
\caption{Time coverage of blacklists and evolution of malicious activities in our dataset.}%}% \ik{Change the y-axis with "Volume of Mal. Activities"}} 
\label{fig:evolution}
\end{figure}


%\begin{figure*}
%\centering
%\includegraphics[width=1\textwidth]{plots/year_wise_malware_distribution_plot.pdf}
%\caption{Analysis of MDL - Yearly Distribution of Reported Malware in MDL.}
%\label{fig:mdl_malware_evolution1}
%\end{figure*}

%Using historical snapshots of the collected dataset, we characterize the behavior of attacks over time? Repeat steps the analysis presented in Section~\ref{sec:characterization} as a function of time.  \ben{Not sure if this statement is relevant/referencing the correct location anymore}
%\begin{itemize}

%\subsection{Internet Attacks Behavior}
%We shed lights on the behavior of reported Internet attacks. We analysis the dropouts, additions, churn, and persistency of reported attacks in our dataset. 
%\subsubsection{Dropouts} – the malware that never returned or cleaned for ever
%\subsubsection{Additions} – the malware that are added to the list
%\subsubsection{Churn} - what is the magnitude and rate of attacks churn? 

%\subsection{Temporal Analysis of Malicious Activities}
%\ben{Pending rework of results, do not analyze yet.}
%\beri{Section 6.2 and 6.3 skipped as the results are not final + the text is lacking insight}
%%\ik{Retitle this subsection with some meaningful title.}
%
%In this Section, we aim perform temporal analysis of malicious activities. 
%%
%%Continuing with Entropy as a tool, we now focus on the Time distribution of the Attack types.
%%
%To this end, we introduce these notions:
%\begin{enumerate}
%   \item Homogeneity of Time Bins
%   \item Time-stability of classes of malicious activities
%   \item Evolving time-stability of classes malicious activities
%\end{enumerate}
%
%%%%%%%%%%
%% Analysis 1
%%\subsubsection{Homogeneity of Time Bins}
%{\bf Homogeneity of Time Bins. }
%In this first analysis we investigate the homogeneity of attacks in time bins, this translates to knowing for a specific time window, how distributed are the contributing reports over the different classes of malicious activities. We will be varying the size of these time windows to the degree of Days, Weeks and Months.
%%
%\begin{figure}[H]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/Time-Attk-combined-Entropy_CDF.pdf}
%\caption{Temporal analysis of all malicious activities: CDF of our time frames on the entropy of a malicious activity class's diversity \ben{pending rework}} 
%\label{Fig:results:time_daily_by_attk_cdf}
%\end{figure}
%%
%To proceed, with Equation \ref{eqn:norm_shannon}, we define $P(n)$ as the probability of selecting a class of malicious activity ($n$) from the aggregated reports of the $i^{th}$ time bin.
%
%In Figure \ref{Fig:results:time_daily_by_attk_cdf}, 
%we can see the Distribution of the attacks types within each time window. From the plot we observe that there is a fairy consistent spread for the time frames with any amount of attacks. But we note that 20\% of the daily frames  contained only one type of malicious activity. but this is not observed in the lower resolution time frame of the weeks and months evidenced in the left hand side of the x-axis approaching 0 CDF.
%
%%%%%%%%%%
%% Analysis 2
%%\subsubsection{Time-Stability of Attack Classes}
%{\bf Time-Stability of Malicious Activities}
%Next, we focus on a specific class of malicious activity. In essence, we aim to analyze the affinity (cf. Section~\red{xref}) of specific class of malicious activity to a particular number of monthly windows. Thus providing an insight into what kind of temporal behavior in a specific class of malicious activities in our dataset. In particular, we are interested to observe (if any) bursts of malicious activity--meaning low entropy values in certain windows of time i.e., days, weeks, or moths--as opposed to a class of malicious activities that remains evenly distributed over time. 
%
%%The Second analysis presented here is an extension of the previous point, but with a focus on a specific attack class. It aims to display an attack type's affinity to a particular number of monthly windows. Thus providing an insight into what kind of temporal behavior is present in an attack as an entity. And thus we should be able to observe bursty activity as having a lower entropy as the Entropy will be dominated by a few key time windows as opposed to an attack class that is consistently propagating in time.
%
%In Equation \ref{eqn:norm_shannon}, We define $P(n)$ as the probability of selecting a time bin ($n$) from the collective reports of the $i^{th}$ malicious activity class.
%
%Table \ref{tab:attack_time_affinity} shows the results of this analysis. We observe the extremely low value of entropy in the Phishing attack class is caused by the influx of live reports as provided by OpenPhish~\cite{openphish} and not because phishing attacks are very lumpy within time. 
%
%\begin{table}[ht!]
%\centering
%\scriptsize
%%\vspace{-0.5cm}
%\begin{tabular}{ rrrrrrrr }
%\toprule
%\midrule
%{\bf Metric} & {\bf PUP} & {\bf FS} & { \bf Malware}&{\bf Exploits}&{\bf Phishing} &{\bf Spammers}&{\bf Total}\\
%\midrule
%Affinity & 0.748& 	0.706& 	0.745& 	0.784	& 	0.0863& 	0.688& 	\ik{xx}\\
%\bottomrule
%\end{tabular}
%\caption{The affinity--normalized Shannon,$H_{n}$, cf. Section~\ref{subsec:entropymetrics}--of malicious activities observed over monthly time windows. \ben{pending rework} }
%\vspace{-0.5cm}
%\label{tab:attack_time_affinity}
%\end{table}
%
%%%%%%%%%%
%% Analysis 3
%%\subsubsection{Evolving Time-Stability of Attack Classes}
%{\bf Evolving Time-Stability of Malicious Activities. }
%To uncover additional information about the changing affinities of the classes of malicious activities over time, we use a sliding window approach, in which the window is then binned into time bins, to entropy as function of sliding window over time bin. 
%%In this analysis in this configuration further extends what was presented in the previous analysis, whilst the previous analysis was taken over the entire time-period, we desired to uncover additional information about the changing affinities of the classes of malicious activities over time. And thus we implement a sliding window approach, in which the window is then binned into time bins, effectively obtaining a value of entropy as this windows slides over every time bin.
%
%In Equation \ref{eqn:norm_shannon}, we define $P(n)$ as the probability of selecting a time bin ($n$) from the collective reports of the $i^{th}$ class of malicious activities in a given sliding window.
%
%Figure \ref{Fig:results:time_month_by_attk_heat} highlights the results of our analysis. From the heatmap we are able to differentiate between the classes of malicious activities that there has been period of burst of malicious activities as indicated by the lighter regions (lower values of entropy). We note that if there are no reports in a time window, the value of entropy will also be 0.
%
%\begin{figure}[H]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/Time-Attk-monthly-Entropy-Heatmap.pdf}
%\caption{Temporal Analysis of Classes of Malicious Activities: Heatmap of our Monthly-Year sliding windows on the entropy of Time Diversity for each attack type.\ben{pending rework}} 
%\label{Fig:results:time_month_by_attk_heat}
%\end{figure}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Hosts - Time
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Temporal Analysis of Malicious Hosts}
%In this Section, we focus on analyzing the temporal behavior of Hosts that correspond to different classes of malicious activities. We aim to illuminate on hosts stability from three vantage points: stability in all malicious activities, stability with respect to specific class of malicious activities, and evolving stability over time. 
%
%\ben{Pending rework of results, do not analyze yet.}
%
%{\bf Overall Stability of Malicious Hosts. }
%One last configuration we wish to investigate is the behavior of the Hosts over time, malicious activity class agnostic. For every host a value of entropy is obtained, describing the host's affinity to a specific time bin. Effectively describing the stability of Host's behavior across its active time bins. 
%%
%In Equation \ref{eqn:norm_shannon}, we define $P(n)$ as the probability of selecting a time bin ($n$) from the collective reports of the $i^{th}$ Host.
%
%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/IP-Time-Entropy_CDF.pdf}
%\caption{Temporal Analysis of Host (i.e., IPs): CDF of our IP on the entropy of Monthly Time Diversity for each IP\ben{pending rework}}
%\label{Fig:results:IP_by_time_cdf}
%\end{figure}
%
%Figure \ref{Fig:results:IP_by_time_cdf} show the result of our analysis.  14\% of the overall IPs (14\%) appear in more than one time bin that suggests that these IPs involve in more than one malicious activities.
%Approximately 86\% of all IPs (Hosts) only exhibit behavior in only one time bin, indicating a high presence of one-time offenders. 
%%%%%%%%%%
%% Analysis 2
%%\subsubsection{Time-Stability of Attack Class Hosts}
%
%{\bf Stability of Hosts in a Specific Class of Malicious Activities.}
%%{\bf Time-Stability of Attack Class Hosts}
%We further extend this analysis by repeating this analysis with the subsets of Hosts within the different classes of malicious activities. We use the same definition of stability, however, perform analysis of each class of malicious activities. 
%
%
%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/IP-Time-Entropy-CDF-separate-Attacks.pdf}
%\caption{Temporal Analysis of Host (i.e., IPs): IP on the entropy of Monthly Time Diversity for each IP, separated into Attack Types\ben{pending rework}}
%\label{Fig:results:IP_by_time_attack_cdf}
%\end{figure}
%
%Figure \ref{Fig:results:IP_by_time_attack_cdf} shows the result of our analysis. Compared to other classes of malicious activities, 9\% of the IPs that correspond to malware class of malicious activities are recurrent offenders i.e., involved in more than one activity within the malware class of malicious activities. Similarly, 3\% and $1\%$ of IPs that correspond to fraudulent services and PUP are involved in more than one malicious activity within their respective classes of malicious activities. For all other classes of malicious activities, all of their IPs are only one time offenders. Overall, our analysis suggests that all large fractions of IPs that belong to different classes of malicious activities are only one time offenders. 
%
%%are Approximately 86\% of all IPs only exhibit behavior in one time bin, indicating a high presence of one-time offenders.
%
%%%%%%%%%%
%% Analysis 3
%%\subsubsection{Evolving Time-Stability of Hosts}
%{\bf Evolving Stability of Hosts. }
%Now, we turn our analysis to investigate the temporal changes in Hosts' affinities. We use a sliding window approach to measure the affinity of hosts over time. 
%%In this analysis, extend what was presented in the previous analysis, whilst the previous analysis was taken over the entire time-period, we aim to uncover additional information about the changing affinities of the hosts classes over time. 
%%And thus we implement a sliding window approach, in which the window is then binned, effectively obtaining a value of entropy as this windows slides over every time bin.
%%
%In Equation \ref{eqn:norm_shannon}, we define $P(n)$ as the probability of selecting a time bin ($n$) from the collective reports of the $i^{th}$ host within the defined sliding window.
%
%%\ik{As we cannot use the same heatmap format as before currently is an average +- STD, this is probably not the optimal way of viewing this result.}
%
%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/Entropy-CDF-separate-Attacks_weekly_entropies.pdf}
%\caption{Temporal Analysis of Host (i.e., IPs): IP on the entropy of Weekly Time Diversity for each IP, separated into classes of malicious activities. \ben{pending rework}}
%\label{Fig:results:IP_by_time_attack_week_cdf}
%\end{figure}
%
%Figure~\ref{Fig:results:IP_by_time_attack_week_cdf} shows the results of our analysis. We observe the changing behaviors of the hosts over time, we note the time periods in mid-2007 and mid-2012 as having higher averages than normal, which could infer that there was increased consistency of time-activity during this time. Another thing to concern ourselves with is the differences in the gradients of increasing entropy, and the sudden decrease in activity. The behavior at the end of the plot near 2017, is due to the window 'Running out of data' to process, thus skewing the final results, to resolve this we need to restrict where the sliding window finishes.
%
%
%Summary:
%These analyses alone does provide information about how consistent the infection is; however does not provide any information about the exact lifetimes or severity of these Hosts, and will be investigated in a later section. \red{Critical TODO: There are still variants of this skew to be run on ASNs and CCs}
%
%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/yearly-IP-Time-Entropy_stats.pdf}
%\caption{IP-Time Analysis: Distribution of IP Specific activity over Year-long monthly windows\ben{pending rework}} 
%\label{Fig:results:IP_by_time_statistics}
%\end{figure}
%
%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/yearly-ASN-Time-Entropy_stats.pdf}
%\caption{ASN-Time Analysis: Distribution of ASN Specific activity over Year-long monthly windows\ben{pending rework}} 
%\label{Fig:results:ASN_by_time_statistics}
%\end{figure}


\subsection{Stability of Hosts and Malicious Activities}

{\bf Stability.} To measure the spread of a given host and/or class of malicious activity (cf. \S~\ref{sec:mtypes}) across reported weekly time bins. we define \emph{Stability} as the normalized Entropy per host and/or malicious activity $i,a$ as $A(a) = (-\sum_{\forall h} P(h) \log_2{P(h)})/\log_2 k$ where;
\begin{equation} \label{eqn:attack_affinity}
P(h) = \frac{\# \, \text{of reports from host $h$ and/or activity $a$ in time bin $t$}}{\text{Total} \, \# \, \text{of reports for host $h$ and/or activity $a$}}
\end{equation}
In this regard, $A(i,a)=1$ represents that reports of host and malicious activity $i,a$ are evenly distributed among all time bins and conversely $A(a)=0$ represents that all reports are concentrated on a single instance of time. 



From the Entropy Equation, for Stability we define $P(n)$ as the probability of selecting a time bin ($n$) from the collective reports of the $i^{th}$ Host.

Figure \ref{Fig:results:stability_host} shows the results of this analysis, from the long head of all distributions, that a large portion of hosts them to either be one time offenders (IP-65.9\%, ASN-29.4\%, CC-7.1\%), in particular with IPs.

With the Stability separated into specific classes of malicious activities, we define $P(n)$ as the probability of selecting a time bin ($n$) from the collective reports of the $i^{th}$ IP for a specific Attack type..

Figure \ref{Fig:results:stability_attacks} shows the results of this analysis, from the long head of all distributions, that a large portion of IPs regardless of attack type are one time offenders, Malware has the least one time offenders of all the attack types.



Below in Table \ref{tab:ip_stability} is the results for the Stability of a class of malicious activity independent of host, focusing solely on the type of activity, there is no point in aggregating into higher levels of hosting infrastructure, as the number of reports per time bin will remain the same even after aggregation. It is truly independent of host. But from this table, we can observe that Fraudulent Services is slightly less homogenous than the others, and Phishing is slightly more homogenous in it's behaviors.


\begin{table}[h!]
\centering
\scriptsize
\begin{tabular}{ rrrrrrrr }
\toprule
\toprule
{\bf Metric} & {\bf PUP} & {\bf FS} & { \bf Malware}&{\bf Exploits}&{\bf Phishing} &{\bf Spammers}&{\bf Total}\\
\midrule
Stability &  0.822 & 0.795 & 0.847& 0.819& 0.894& 0.853& 0.848\\
\bottomrule
\end{tabular}
\caption{Stability of Hosts in our dataset.}
\label{tab:ip_stability}
\vspace{-0.2cm}
\end{table}


\begin{figure}[ht!]
\centering
\subfloat[\small Hosts]{\includegraphics[width=0.49\columnwidth]{./new_plots/stability_hosts_CDF.pdf}
\label{Fig:results:stability_host}}
\subfloat[\small Classes Malicious Activities]{\includegraphics[width=0.49\columnwidth]{./new_plots/stability_attacks_CDF.pdf}\label{Fig:results:stability_attacks}}
\caption{Stability Analysis: Distribution of Stability for Hosts (Figure \ref{Fig:results:stability_host}) and classes of Malicious activities (Figure \ref{Fig:results:stability_attacks})} 
\label{Fig:results:stability}
\end{figure}


\begin{figure}[ht!]
\centering
\subfloat[\small Hosts]{\includegraphics[width=0.49\columnwidth]{./new_plots/churn_severity_mean_weekly.pdf}\label{Fig:results:tier_by_severity_cdf_wk}}
\subfloat[\small Classes Malicious Activities]{\includegraphics[width=0.49\columnwidth]{./new_plots/churn_attack_severity_mean_weekly.pdf}\label{Fig:results:attack_by_severity_cdf_wk}}
\hspace{-0.3cm}
\caption{Severity Analysis: Mean Normalized Severity of Hosts (Figure~\ref{Fig:results:tier_by_severity_cdf_wk}) and classes of Malicious activities (Figure~\ref{Fig:results:attack_by_severity_cdf_wk}).}% \beri{We need a zoom here for the values between 1 and 10} \ben{xlimed to 100 for attacks, because of funky looking country curve. Looks even cooler on the scatter plot Figure \ref{Fig:results:sev_life} and \ref{Fig:results:sev_death}}} 
\label{vt:severity:analysis}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Churn Analysis 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Churn Analysis}
\label{sec:churn}

%In this section we focus in on the time-behavior of out dataset, attempting to find trends and relationships in time. We will be elaborating on our definitions of Hosts being 'Alive', as well as leveraging Autocorrelation in order to extract trends from the dataset \ben{The Autocorrelation has currently been excluded, not sure how to extract meaning besides pointing out lag 30 is statistically significant (monthly trends)}. We extend Yao et al.,~\cite{Yao:ICNP:2006}'s Churn model where they have presented a churn model as a binary function of either Alive(1) or Dead(0) of a participating ``peer'' in a system. We now take their original definition of Churn and modify the Alive status to take a value $k$, to represent the number of reports that has occurred within this time bin. This modification allow the model to capture the Liveliness or Severity of the Host.

To understand the dynamics of churn of malicious actors, we start by creating a model of host behavior
and specifying assumptions. The focus of this section is to formalize recurring hosts participation in malicious activities in a simple model as well as to explain the relationship between the various lifetime distributions observable in these networks. 

{\bf The model: } Consider a malicious ecosystem with $n$ participating hosts, where each host $i$ is either alive (i.e., present in the system) at time $t$ or dead (i.e., logged off/clean). At any time $t$, an active host can be reported one or multiple times as being malicious (denoted $k$). This behavior can be modeled by an alternating renewal process ${Z_i(t)}$ for each host $i$ similar to Yao et al.,~\cite{Yao:ICNP:2006}'s Churn model :

\begin{equation}
  Z_i(t) =
  \begin{cases}
    \multirow{2}{*}{$K$,} & \text{host $i$ has receieved}\\
                                    & \text{$K$ reports at time $t$}\\
    0, & \text{Otherwise}
  \end{cases}
  , 1\leq i \leq n
\end{equation}

where $n$ is the total number of hosts in our dataset and $t$ is in weeks. Hence, our trace is created by binning the reports by weeks and per participating entity.

%\beri{a sentence or two on how we build the traces} 
%\ben{We build our traces by binning the reports into weeks as defined in ISO week date system, each bin will contain the aggregate of the Entity's reports during that week - $k$.}


\begin{figure}[ht!]
\centering
\includegraphics[width=1\columnwidth]{./imgs/Churn_Model.pdf}
\caption{Churn Model representing Life and Severity. $K_{i,c}$ is the total number of reports in the $c^{th}$ period (i.e., week) of activity of Host $i$.}%  \ben{$K_{i,c}$ refers to the Area under the curve} \ben{I'm not sure if my diagram notation is right, should i have $k$ where the upwards arrow at $t$ is?, so should it remain $Z_i(t)$}} 
\label{Fig:churn_model}
\end{figure}


%
%From the original P2P paper we retain their original definitions of Mean Lifetime, Deathtime, and the Reciprocal of mean Life and Death:
Our model is illustrated in Figure ~\ref{Fig:churn_model} where variable $c$ stands for the cycle number and durations of user $i$'s ON (life) and OFF (death) periods are given by random variables $L_{i,c}$ > 0 and $D_{i,c}$ > 0, respectively.

%\beri{Still don't know what kic means in Fig 19 and the whole explanation is not satisfactory. Maybe an example or get rid of the plot?} 
%\ben{For $K_{i,c}$ definition, see comment in section \ref{sec:severity}. But as a brief sentence: $K_{i,c}$ is the total number of reports within the $c^{th}$ period of activity of host $i$ (aka area under the curve) (If you considered Figure \ref{Fig:churn_model}, and treated every step as 1 report, and every horizontal change 1 week, for time period $c+1$, we would have a total of 9 reports, over a time period of 5 weeks.  Severity = $K_{i,c} = 9 reports$,  Normalised severity = 9/5 reports per week)}
%\ben{$i$ denotes the specific entity currently being tracked in time, $c$ denotes the cth occurence of consecutive time time-bins marked as containing malicious activity. Lower case indicates the mean value across all c occurrences, whilst Upper case is related to the specific cth value}

%\beriw{Yao et al.,~\cite{Yao:ICNP:2006} made several assumptions among which that users behave independently of
%each other. This is not TRUE in our scenario as for example botnets are a coordinated attack. I don't know how this would %affect the findings}
%\ben{On Yao's first assumption, "This assumption also implies that users simultaneously present in the system with multiple identities are not very common and have no large-scale impact on the dynamics of the network", this allows Yao to create an independent random processes for each user, Would it not be a problem, as we are using this definition to report metrics, as opposed to re-simulating it's behavior. i.e. if we were to replay this behavior, we should evaluate another model}

%\ben{Second assumption of the joint probability between $L$ and $D$ is not an assumption, but is true in our case, as if an entity is alive, it cannot dead}
%\ben{I would argue that we are only using this model to just present the information within our dataset, and the assumptions will not affect this empirical presentation, these assumptions can be regarded as more impactful on the results if we were trying predict future behaviors / simulate the system's behavior}

We adopt the same modeling assumptions as in ~\cite{Yao:ICNP:2006} and assume that all lifetime (i.e., ${\{L_{i,c} \}_{c=0}^\infty}$) and offtime (i.e., ${\{D_{i,c} \}_{c=0}^\infty}$) are \textit{i.i.d. sets of variables}. For convenience of notation, we define the average lifetime as
\begin{equation}
  L_i = E[\{ L_{i,c} \}_{c=0}^\infty]
  \label{Eqn:life}
\end{equation}

and the average offline (or clean) duration as
\begin{equation}  
  D_i = E[\{ D_{i,c} \}_{c=0}^\infty]
  \label{Eqn:death}
\end{equation}


%\ik{explain the literals in equation.}


%The average life of a host is defined as the mean of all the periods of reported activity, each period of reported activity will be separated by a period of inactivity, otherwise it is considered the same period of activity.
%
%A different model for lifetime of a Host as previously been presented within this whereby the Lifetime was taken as the time difference between the time it was first seen, to the time it was last seen. This definition however is not suitable for tracking periods of inactivity within the timeline hosts behavior. Instead with our new definition by considering malicious activity in weekly time blocks, whereby a block is marked as Alive if the number of reports $k > 0$ from the host within the week.
%
%%Where the Life and Death times of the entity may be defined, for the purposes of utilizing this provided model, we first consider the Churn of ASNs independent of attack type, which will be expanded to later on. We define lifetime differently to before, where previously we defined Life Time as the period of time from first reported to last reported as the Alive time, this is unsuitable for the provided definition, due to lack of a statistical inference from the dataset, we have one single time and that's it, no statistical representation e.g. Mean.
%
%
%From this definition we apply the model and obtain the 3 previously proposed metrics, Reciprocal of Mean Duration, Mean Live Time, Mean Death Time, seen in Figures \ref{Fig:results:tier_by_recip_cdf_wk}, \ref{Fig:results:tier_by_life_cdf_wk}, \ref{Fig:results:tier_by_death_cdf_wk}. \ben{Mean life time and Mean Death time are self-explanatory, however with Reciprocal of Life, Death as quoted from Yao's original paper, is "interpreted as the average arrival (or departure) rate of user i."}
Note that long average lifetime depicts entities that are \textit{persistent} (or bulletproof) as their participation in malicious activities is not disturbed for a long time even though they are know for being malicious. On the other hand, low average death depicts \textit{resiliency} as it shows that a malicious entity can quickly recover from a shutdown.

\textbf{Reciprocal of mean duration. }
The Reciprocal of mean duration is representative of the \textit{rate of arrival} of a particular entity. It can be thought of as how frequently this entity participate (or leave) a class of malicious activity and is defined as:
\begin{equation}
  \lambda_i = \frac{1}{l_i + d_i}
  \label{Eqn:recip}
\end{equation}

%We now provide examples for  high and low values of this metric. When an entity is frequently joining and leaving the malicious state, then it is expected that it will have a low average lifetime and also a low average death-time, thus  employing Equation \ref{Eqn:recip}, we will have a larger resulting value from the smaller denominator value. Oh the other hand an entity with a low degree of activity (in joining and leaving) will have either a large mean lifetime or a large mean death-time, resulting in a small value (large denominator) for the reciprocal of mean duration (rate of Arrival).

Consider a scenario where a malicious host is frequently joining and leaving a group of botnet (i.e., in burst), then both average lifetime and average death-time would be small. According to Equqtion~\ref{Eqn:recip}, $\lambda_{i}$ would be large as the value of the dominator would approach zero. Inversely, an entity with a low degree of activity (in joining and leaving) will have either a large mean lifetime or a large mean death-time, resulting in a small value (large denominator) for the reciprocal of mean duration (rate of Arrival).   



\begin{figure}
\centering
\subfloat[\small ]{\includegraphics[width=0.5\columnwidth]{./new_plots/churn_life_mean_weekly.pdf}\label{Fig:results:tier_by_life_cdf_wk}}
\subfloat[\small ]{\includegraphics[width=0.5\columnwidth]{./new_plots/churn_death_mean_weekly.pdf}\label{Fig:results:tier_by_death_cdf_wk}}\quad
\subfloat[\small]{\includegraphics[width=0.5\columnwidth]{./new_plots/churn_reciprical_life_mean_weekly.pdf}\label{Fig:results:tier_by_recip_cdf_wk}}
%\hspace{-0.3cm}
\caption{Churn Analysis: CDFs of mean lifetime, mean deathtime and reciprocal of mean duration (IPs, ASNs, and Countries)} 
\label{vt:churn:hosts}
\end{figure}

Figure \ref{vt:churn:hosts} shows the CDF of mean lifetime, mean death-time and reciprocal of mean duration per IP, ASN and country. The top figure shows that 80\% of the IPs are one time offenders (blue line) with an average duration of just a week. This number decreases dramatically if we consider ASN (55\%) or country (20\%). The long tail for both IP and ASN indicates that few entries have a much longer lifetime duration. We list top-10 IPs, ASNs, and countries in Table~\ref{tab:ldarrival:analysis}.   91.193.194.114 and AS4134 are reported as malicious for 25 and 35.2, respectively, consecutive weeks. 

The results in Figure~\ref{vt:churn:hosts} and Table~\ref{tab:ldarrival:analysis} suggest that while at micro level (i.e., IP) malicious entity lifetime is relatively small, at a macro level (ASN and country) this is not the case. When looking at the mean death time, Figure~\ref{Fig:results:tier_by_death_cdf_wk} and Table~\ref{tab:top_death}, a similar conclusion can be drawn. At a micro level, most IPs have a mean death time bigger than 100 weeks indicating a single participation while the ``long head'' indicates that few hosts are recurring participants. At a macro level, however, the mean death time is greatly decreased indicating that most ASN and countries are repeating offenders.


At a country level and from a resiliency view point, the USA is ranked first with the smallest average death time of $0.01$ weeks followed by Germany (1.47) and British Virgin Islands (1.61). China, Ukraine, and Great Britain are the most persistent countries with the longest average lifetime of 43.8, 29.6 and 27.8 weeks\footnote{The observation period is in week, starting from 2007 to 2017.}, respectively. These results show that countries with the largest number of connected users dominate the offender list.

However, the picture would not be entirely complete if we do not shed light on smaller countries (i.e., in term of connected users). To do so, we computed the rate of arrival and ranked the countries accordingly. In Table~\ref{tab:top_arrival}, the top 3 are Panama, Bahamas and Colombia with arrival rates of 0.15, 0.14 and 0.14, respectively. This shows that aggregate results that only take volumes in account usually fail to depict a complete picture of the threat landscape by ignoring \textit{emergent} actors. 

\begin{figure}[ht!]
\centering
\subfloat[\small Mean Lifetime]{\includegraphics[width=0.5\columnwidth]{./new_plots/churn_attack_life_mean_weekly.pdf}\label{Fig:results:attm_by_life_cdf_wk}}
\subfloat[\small Mean Deathtime]{\includegraphics[width=0.5\columnwidth]{./new_plots/churn_attack_death_mean_weekly.pdf}\label{Fig:results:attk_by_death_cdf_wk}}\quad
\subfloat[\small Reciprocal of mean duration]{\includegraphics[width=0.5\columnwidth]{./new_plots/churn_attack_reciprical_life_mean_weekly.pdf}\label{Fig:results:attk_by_recip_cdf_wk}}
\subfloat[\small Legend]{\includegraphics[width=0.5\columnwidth]{./plots/eplots/attk_legend.pdf}\label{Fig:results:attk_legend}}
\caption{Churn Analysis: CDFs of Reciprocal of mean duration, mean Lifetime, and mean Deathtime for Malicious Activities }%\ben{Fix legend plot, delete this set if no conclusions can be drawn}} 
\label{vt:churn:attacks}
\end{figure}
%\beriw{What is the observation period... What is the max in the plot? 100 weeks more less??}
%\ben{The observation period is in week, starting from 2007 to 2017}%, to put into perspective country LR has a death-time of 536 weeks}

%\beri{We need some text to explain the plots above. We cannot directly jump to extreme values. Why more than 90\% have an average lifetime equal to zero?}
%\ben{>90\% of samples have $10^0 = 1$ lifetimes, in this case the 1 week time bin. i.e. they are the one time offenders}
%\textbf{Extremity Examples}

%We can describe entities that have a long average lifetime as being persistent with their participation in malicious activities, as there are no breaks between their activity. On the other hand the entities which have a very low average deathtime can be regarded as being resilient in the sense that whence their malicious activity has ceased, they are very quick to start participating within the malicious activity again.
 
%From these descriptors, we can describe China has having the most persistent behavior, with it's long average lifetime of 43.8 weeks, however with a deathtime of 9.9 weeks, whence compared to the United States with an average deathtime of 1.28 Weeks, the United States is the most resilient participant of malicious activities.

%\ben{
%Related to Figure \ref{Fig:results:tier_by_life_cdf_wk}, the longest period of consecutive weeks of malicious activity is carried out by ip: 91.193.194.114, for 25 weeks without any death-time as defined by by our churn model. Whence aggregated into the ASN Level, AS4134 has the longest average lifetime at 35.17 weeks, with a deathtime of 0.5 weeks average. The asn with the shortest avg deathtime is AS26496, with and average 2.0 weeks, and a avg. lifetime of 13.31 weeks. Finally the country (cc) with the longest lifetime of malicious activity is China (CN) with an average of 43.8 weeks of activity, however having a much longer average deathtime of 9.9 weeks. We contrast this with the country with the shortest average deathtime, the United States (US) with an avg. deathtime of 1.28 weeks, but a shorter average lifetime of 20.2 weeks. }

%\textbf{Reciprocal of mean duration}
%Table \ref{tab:top_arrival} we can quickly view the top 10 entities from IP, AS, CC in therms of rate of arrival.

\begin{table*}[ht!]
\centering
\scriptsize
%\small
\tabcolsep=0.040cm
\subfloat[Average Lifetime (Most Persistent)]{\label{tab:top_life}\scalebox{1.0}{
\begin{tabular}{ r c r| c c r| c c r }
\toprule
{\bf IP}	&	{\bf LT}	&	{\bf AVS.}	&	{\bf ASN}	&	{\bf LT}	&	{\bf AVS.}	&	{\bf CC}	&	{\bf LT}	&	{\bf AVS.}\\
\midrule
91.193.194.114	&	62	&	\red{x}	&	3257	&	55	&	80\%	&	US	&	511	&	79\%	\\
109.86.226.85	&	52	&	\red{x}	&	9800	&	38	&	-	&	RU	&	33	&	47\%	\\
68.70.242.203	&	48	&	\red{x}	&	35994	&	23	&	80\%	&	DE	&	29	&	74\%	\\
212.227.247.242	&	38	&	\red{x}	&	46514	&	23	&	-	&	NL	&	27	&	72\%	\\
87.249.142.189	&	37	&	\red{x}	&	34040	&	22	&	-	&	GB	&	25	&	58\%	\\
89.163.139.243	&	37	&	\red{x}	&	8025	&	21	&	-	&	UA	&	23	&	57\%	\\
85.248.2.228	&	32	&	\red{x}	&	56356	&	20	&	-	&	FR	&	21	&	70\%	\\
178.210.131.104	&	31	&	\red{x}	&	4134	&	20	&	78\%	&	CA	&	19	&	58\%	\\
85.135.104.170	&	29	&	\red{x}	&	38895	&	18	&	57\%	&	CN	&	19	&	78\%	\\
162.249.2.136	&	27	&	\red{x}	&	12604	&	18	&	-	&	KR	&	14	&	68\%	\\

%91.193.194.114  & 25.0 & 4134  & 35.2 & CN & 43.8 \\
%109.86.226.85   & 23.0 & 25190 & 26.0 & UA & 29.6 \\
%68.70.242.203   & 23.0 & 49469 & 26.0 & GB & 27.8 \\
%212.227.247.242 & 23.0 & 46514 & 23.0 & CA & 24.7 \\
%87.249.142.189  & 22.0 & 34040 & 22.0 & BR & 23.4 \\
%89.163.139.243  & 22.0 & 8025  & 21.0 & TR & 23.0 \\
%85.248.2.228    & 21.0 & 24940 & 20.6 & NL & 22.9 \\
%178.210.131.104 & 21.0 & 56356 & 20.0 & RU & 22.9 \\
%85.135.104.170  & 21.0 & 16276 & 19.9 & US & 20.2 \\
%162.249.2.136   & 20.0 & 12604 & 18.0 & DE & 19.2 \\
\bottomrule
\end{tabular}
}}\qquad
%\caption{Table of top 10 Entities with highest Average Lifetime (Most Persistent)}
%\label{tab:top_life}
%\end{table}
\subfloat[Average Deathtime (Most Resilient)]{\label{tab:top_death}\scalebox{1.0}{
\begin{tabular}{ r c r| c c r| c c r }
\toprule
{\bf IP}	&	{\bf DT}	&	{\bf AVS.}	&	{\bf ASN}	&	{\bf DT}	&	{\bf AVS.}	&	{\bf CC}	&	{\bf DT}	&	{\bf AVS.}	\\
\midrule
103.224.212.222	&	3	&	\red{x}	&	36351	&	1.5	&	51\%	&	US	&	0	&	79\%	\\
69.172.201.153	&	3	&	\red{x}	&	26496	&	1.6	&	79\%	&	DE	&	1.5	&	74\%	\\
204.11.56.48	&	4	&	\red{x}	&	40034	&	1.6	&	91\%	&	VG	&	1.6	&	94\%	\\
208.73.211.70	&	4	&	\red{x}	&	13335	&	1.7	&	78\%	&	FR	&	1.7	&	70\%	\\
72.52.4.119	&	4	&	\red{x}	&	14618	&	1.8	&	71\%	&	AU	&	1.9	&	53\%	\\
72.52.4.120	&	5	&	\red{x}	&	21740	&	1.9	&	90\%	&	NA	&	2	&	52\%	\\
54.72.9.51	&	5	&	\red{x}	&	16276	&	1.9	&	71\%	&	PL	&	2.7	&	59\%	\\
185.53.179.8	&	5	&	\red{x}	&	133618	&	2.1	&	83\%	&	SE	&	2.8	&	69\%	\\
213.186.33.19	&	5	&	\red{x}	&	16509	&	2.1	&	85\%	&	NL	&	2.8	&	72\%	\\
8.5.1.51	&	5	&	\red{x}	&	13768	&	2.2	&	73\%	&	RO	&	2.8	&	28\%	\\
%IP              &    Deathtime      & AS    &   Deathtime       & CC &     Deathtime    \\
%\midrule
%103.224.212.222	&	2.97	&	36351	&	1.54	&	US	&	0.01	\\
%69.172.201.153	&	3.1	&	26496	&	1.62	&	DE	&	1.47	\\
%204.11.56.48	&	3.68	&	40034	&	1.63	&	VG	&	1.61	\\
%208.73.211.70	&	4.14	&	13335	&	1.69	&	FR	&	1.7	\\
%72.52.4.119	&	4.14	&	14618	&	1.8	&	AU	&	1.95	\\
%72.52.4.120	&	4.72	&	21740	&	1.89	&	NA	&	1.98	\\
%54.72.9.51	&	4.83	&	16276	&	1.93	&	PL	&	2.74	\\
%185.53.179.8	&	4.87	&	133618	&	2.12	&	SE	&	2.81	\\
%213.186.33.19	&	5.21	&	16509	&	2.15	&	NL	&	2.82	\\
%8.5.1.51	&	5.26	&	13768	&	2.21	&	RO	&	2.84	\\
\bottomrule
\end{tabular}
}}\qquad
%\caption{Table of top 10 Entities with lowest Average Deathtime (Most Resilient)}
%\label{tab:top_death}
%\end{table}
%\begin{table}[]
%\centering
\subfloat[Rate of Arrival (Most Frequently Active)]{\label{tab:top_arrival}\scalebox{1.0}{
\begin{tabular}{ r c r| c c r| c c r }
\toprule
{\bf IP}	&	{\bf RoA}	&	{\bf AVS.}&	{\bf ASN}	&	{\bf RoA}	&	{\bf AVS.}	&	{\bf CC}	&	{\bf RoA}	&	{\bf AVS.}\\
\midrule
69.172.201.153	&	0.18	&	\red{x}	&	8001	&	0.17	&	71\%	&	PA	&	0.15	&	26\%	\\
103.224.212.222	&	0.18	&	\red{x}	&	13649	&	0.17	&	71\%	&	BS	&	0.14	&	94\%	\\
208.73.211.70	&	0.17	&	\red{x}	&	11403	&	0.17	&	73\%	&	CO	&	0.14	&	30\%	\\
8.5.1.51	&	0.14	&	\red{x}	&	21219	&	0.16	&	54\%	&	BG	&	0.12	&	55\%	\\
204.11.56.48	&	0.14	&	\red{x}	&	47869	&	0.16	&	55\%	&	GE	&	0.12	&	63\%	\\
213.186.33.19	&	0.14	&	\red{x}	&	20021	&	0.16	&	42\%	&	EU	&	0.12	&	57\%	\\
72.52.4.119	&	0.14	&	\red{x}	&	12322	&	0.16	&	83\%	&	PH	&	0.12	&	35\%	\\
54.85.127.70	&	0.13	&	\red{x}	&	46636	&	0.16	&	58\%	&	KZ	&	0.12	&	48\%	\\
52.204.129.22	&	0.13	&	\red{x}	&	6849	&	0.16	&	19\%	&	HR	&	0.12	&	29\%	\\
185.53.179.8	&	0.13	&	\red{x}	&	31103	&	0.16	&	29\%	&	MX	&	0.12	&	49\%	\\
%IP              &    ArrivalRate      & AS    &   ArrivalRate       & CC &     ArrivalRate     \\
%\midrule
%69.172.201.153	&	0.18	&	8001	&	0.17	&	PA	&	0.15	\\
%103.224.212.222	&	0.18	&	13649	&	0.17	&	BS	&	0.14	\\
%208.73.211.70	&	0.17	&	11403	&	0.17	&	CO	&	0.14	\\
%8.5.1.51	&	0.14	&	21219	&	0.16	&	BG	&	0.12	\\
%204.11.56.48	&	0.14	&	47869	&	0.16	&	GE	&	0.12	\\
%213.186.33.19	&	0.14	&	20021	&	0.16	&	EU	&	0.12	\\
%72.52.4.119	&	0.14	&	12322	&	0.16	&	PH	&	0.12	\\
%54.85.127.70	&	0.13	&	46636	&	0.16	&	KZ	&	0.12	\\
%52.204.129.22	&	0.13	&	6849	&	0.16	&	HR	&	0.12	\\
%185.53.179.8	&	0.13	&	31103	&	0.16	&	MX	&	0.12	\\
\bottomrule
\end{tabular}
}}
\caption{Top 10 IPs, ASes, and Countries (CC) with: (\ref{tab:top_life})  Highest Average Lifetime (LT), (\ref{tab:top_death})  Lowest Average Deathtime (DT), and (\ref{tab:top_arrival}) Highest Rate of Arrival (RoA) }
\label{tab:ldarrival:analysis}
\end{table*}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Severity

\subsection{Severity of Hosts and Malicious Activities} \label{sec:severity}
%In the previous section, we performed Churn analysis to determine hosts' temporal behavior in terms of their contributions to malicious activities. In this section, we perform Severity analysis of Hosts and malicious activities. To this end, we define two metrics: The first metric describes the average number of malicious reports that spanning every $c^{th}$ (see  Figure~\ref{Fig:churn_model}) period of malicious activity.  
In the previous section, we analyzed the churn of malicious entities and showed that the temporal behavior not only differ from one host to another but also when looking at micro versus macro level. In this section, we perform further analysis to quantify the \textit{severity} of the malicious activity. Formally, %$s_i = E \Bigg[\bigg\{ \frac{K_{i,c}}{L_{i,c}} \bigg\}_{c=0}^\infty \Bigg]$  %To do so, we define two new metrics based on our churn model.

%
%\textbf{Mean Severity}: This metric describes the average number of malicious reports for a specific entity per $c^{th}$ period of activity and can be formalized as $S_{mean} = E\big[\{ K_{i,c} \}_{c=0}^\infty\big]$. \beri{As far as I can tell we are not using this metric. If so, it has to be removed}
%\ben{This is not being used anywhere.}

%\ben{Mean Severity is not per week, it is just the average number of reports per $c^{th}$ period of activity, what you are referring to with the reports per week is the Normalized Severity Equation \ref{Eqn:severity}}

\begin{equation}
  \text{s}_{i} = E \Bigg[\bigg\{ \frac{K_{i,c}}{L_{i,c}} \bigg\}_{c=0}^\infty \Bigg],
  \label{Eqn:severity}
\end{equation}

where $K_{i,c}$ is the total number of reports within the $c^{th}$ period of activity (i.e, area under the curve) of host $i$. For instance in Figure \ref{Fig:churn_model}, treat every step of the curve as 1 report and every horizontal change as 1 week then for time period $c+1$, we would then have a total of 9 reports (i.e., $ K_{i,c+1}$ = 9) and a time period of 5 weeks (i.e., $ L_{i,c+1}$ = 5), Therefore, the Severity is equal to 9/5 reports per week (i.e., $s_{i,c+1}$) = 9/5).
%
%The mean severity defined above accumulates the number of reports per host over time and hence is dependent of its lifetime. 
%To overcome this, we define a normalized version by having an observation window (a week) and defined it as $S^n_{mean} = E \Bigg[\bigg\{ \frac{K_{i,c}}{L_{i,c}} \bigg\}_{c=0}^\infty \Bigg]$. 
%
This formalism allows us to distinguish between the two following scenarios: $(i)$ A long-living (persistent) host and $(ii)$ A short-living host with high malicious activity.

%The second form is derived from the first metric where we normalize the metric %to remove time as variable, 
%to measure the expected severity of the host independent of the lifetime of the current period of malicious activity. We formalized this normalized severity as: $S^n_{mean} = E \Bigg[\bigg\{ \frac{K_{i,c}}{L_{i,c}} \bigg\}_{c=0}^\infty \Bigg]$. %Formally: %, Equation \ref{Eqn:severity} notes this definition.
%\begin{equation}
%  \text{Normalized Severity}_{mean} = E \Bigg[\bigg\{ \frac{K_{i,c}}{L_{i,c}} \bigg\}_{c=0}^\infty \Bigg]
%  \label{Eqn:severity}
%\end{equation}
%This normalized metric allows us to differentiate between the following cases: $(i)$ A Long-living (persistent) Host (i.e., IP, ASN, or Country) in time will aggregate reports and thus its severity will be high; and $(ii)$ A Short-living host, but of very high malicious activity will also result in a very high severity.

%In the previous section, we have a definition of Churn allows for an analysis of the number of reports a host has received in a particular time period, we will term this as the Severity of the host, and will come in two different forms. The first metric will factor in both the number of reports and the time interval in which the host was active i.e., the area under the activity curve in Figure \ref{Fig:churn_model}. 
%The second form is derived from the first metric where we normalize the metric to remove time as variable, producing the expected severity of the host independent of the lifetime of the current period of malicious activity. Equation \ref{Eqn:severity} notes this definition. This normalized metric allows the differentiation between the following cases: $(i)$ A Long-living (persistent) Host (i.e., IP, ASN, or Country) in time will aggregate reports and thus its severity will be high; and $(ii)$ A Short-living host, but of very high malicious activity will also result in a very high severity.
%\begin{enumerate}
%\item A Long-living (persistent) Host (i.e., IP, ASN, or Country) in time will aggregate reports and thus its severity will be high.
%\item A Short-living host, but of very high malicious activity will also result in a very high severity.
%\end{enumerate}
%By normalizing over the time the host was active for, we are able to obtain the normalized severity of these hosts, irrespective of the time it's been active. We show the results of our analysis in Figure \ref{Fig:results:tier_by_severity_cdf_wk} and Table \ref{Tab:tiered_spearman}. In Figure \ref{Fig:results:tier_by_severity_cdf_wk}, 60\% of IPs have severity value $1$ whilst 63\% of ASNs and 87\% of countries have severity greater than 1, respectively. Overall, when we analyze malicious activities of hosts at different levels i.e., IP, AS, or country, the severity increases--the number of malicious activity per unit time (here we have one-week as a bin) increases. When we analyze the severity of malicious activities, in Figure\ref{Fig:results:attack_by_severity_cdf_wk}, we notice that Fraudulent services have higher severity when compared to the rest of the classes. However, when we observe the long tail of distributions we found that \red{x\%}, {y\%}, and {x\%} of Exploits, Phishing, and Malware have the severity values at least 100. 
Figure \ref{Fig:results:tier_by_severity_cdf_wk} and Table~\ref{vt:severity:analysis} report the results for the above metric. First, 60\% of IPs have a severity value equal to one indicating a unique malicious report per unit of time. However, at a higher level of abstraction this value decreases to 37\% for ASN and 13\% for country. Second, the long tail for IPs indicates that while most hosts are only reported once, few others are participating in a plethora of malicious activities with \red{(number)} hosts reported thousands of times per week.  Finally, the distribution of both ASN and country indicate that at a macro level, malicious activity has become the norm rather than the exception. These results are consistent with our findings in section \ref{sec:churn}. \beri{Don't like the last two sentences but}

 
\beriw{We need more findings here otherwise we should remove this part. Provided information is somehow redundant with the churn analysis.}

Next, we aim to investigate relationship (if any) between hosts' and malicious activities' severity and their Lifetime as well as Deathtime. In Figure \ref{Fig:results:sev_life} and \ref{Fig:results:sev_death}, there is an obvious trend and relationship between the Normalized Severity and the both the mean Lifetime and men Deathtime, in particular with the countries. We leverage the Spearman Correlation coefficients [\red{cite}], $\rho$, in order to quantify the strength of the relationship observed within these plots. In Table~\ref{Tab:tiered_spearman}, we observe that the longer the hosts' lifetimes the higher the severity (\red{how much}) of it's malicious campaigns irrespective of the length of the campaign (i.e., Severity).   \ik{Tell me more. Add AV-scores. } 

\begin{figure}[ht!]
\centering
\subfloat[\small Severity and Mean Lifetime.]{\includegraphics[width=1\columnwidth]{./new_plots/mean_life_norm_severity_scatter.png}\label{Fig:results:sev_life}}\quad
\subfloat[\small Severity and Mean Deathtiime.]{\includegraphics[width=1\columnwidth]{./new_plots/mean_death_severity_scatter.png}\label{Fig:results:sev_death}}
\caption{Severity Analysis: correlation between Severity and Mean Lifetime/Deathtime. } 
\end{figure}

\begin{figure}[ht!]
\centering
\subfloat[\small Hosts]{\includegraphics[width=0.49\columnwidth]{./new_plots/churn_severity_mean_weekly.pdf}\label{Fig:results:tier_by_severity_cdf_wk}}
\subfloat[\small Classes Malicious Activities]{\includegraphics[width=0.49\columnwidth]{./new_plots/churn_attack_severity_mean_weekly.pdf}\label{Fig:results:attack_by_severity_cdf_wk}}
\hspace{-0.3cm}
\caption{Mean Normalized Severity of IPs, ASes, and Countries (Figure~\ref{Fig:results:tier_by_severity_cdf_wk}); and classes of malicious activities (Figure~\ref{Fig:results:attack_by_severity_cdf_wk}).}% \beri{We need a zoom here for the values between 1 and 10} \ben{xlimed to 100 for attacks, because of funky looking country curve. Looks even cooler on the scatter plot Figure \ref{Fig:results:sev_life} and \ref{Fig:results:sev_death}}} 
\label{vt:severity:analysis}
\end{figure}


\begin{table}[ht!]
\centering
\small
%\scriptsize
\tabcolsep=0.040cm
%\subfloat[ $\rho$ between Normalized Severity and Mean Life]{\label{tab:sp:lt:severirty}\scalebox{1.0}{
\subfloat[ ]{\label{tab:sp:lt:severirty}\scalebox{1.0}{
%\begin{tabular}{R{2cm}C{1.3cm}C{1.3cm}C{1.3cm}}
\begin{tabular}{rccc}
%\begin{tabular}{rccc}
\toprule
   & {\bf $\rho (IP)$} & {\bf $\rho(AS)$}  & {\bf $\rho(CC)$} \\
\midrule
Malware            & 0.282 & 0.506 & 0.623 \\
PUP  & 0.406 & 0.482 & 0.658 \\
Fraud. Serv. & 0.154 & 0.422 & 0.758 \\
Exploits           & 0.254 & 0.505 & 0.674 \\
Phishing           & 0.243 & 0.518 & 0.805 \\
Spammers           & 0.312 & 0.364 & 0.514 \\
Totals             & 0.298 & 0.546 & 0.704 \\
\bottomrule
\end{tabular}
\label{Tab:tiered_spearman}
}}
%\subfloat[$\rho$ between Normalized Severity and Mean Death]{\label{tab:sp:dt:severirty}\scalebox{1.0}{
\subfloat[ ]{\label{tab:sp:dt:severirty}\scalebox{1.0}{
%\begin{tabular}{R{2cm}C{1.3cm}C{1.3cm}C{1.3cm}}
\begin{tabular}{rccc}
\toprule
   & {\bf $\rho (IP)$} & {\bf $\rho(AS)$}  & {\bf $\rho(CC)$} \\
\midrule
Malware            & -0.357 & -0.543 & -0.575 \\
PUP  & -0.403 & -0.482 & -0.714 \\
Fraud. Serv. & -0.142 & -0.380 & -0.670 \\
Exploits           & -0.176 & -0.484 & -0.660 \\
Phishing           & -0.133 & -0.450 & -0.666 \\
Spammers           & -0.313 & -0.421 & -0.734 \\
Totals             & -0.334 & -0.545 & -0.644 \\
\bottomrule
\end{tabular}
\label{Tab:attack_spearman}
}}
\caption{Spearman coefficients ($\rho$) determine the relationship between metrics: (\ref{tab:sp:lt:severirty}) $\rho$ between Normalized Severity and Mean Life; and (\ref{tab:sp:dt:severirty}) $\rho$ between Normalized Severity and Mean Death. }
\label{Tab:spearman}
\end{table}


\begin{table}[ht!]
\centering
%\scriptsize
\small
\tabcolsep=0.040cm
\begin{tabular}{ r c r| c c r| c c r }
\toprule
{\bf IP}	&	{\bf Severity}	&	{\bf AVS.}	&	{\bf ASN}	&	{\bf Severity}	&	{\bf AVS.}	&	{\bf CC}	&	{\bf Severity}	&	{\bf AVS.}\\
\midrule
176.31.26.214	&	3137	&	\red{x}	&	7415	&	771	&	96\%	&	US	&	9218	&	79\%	\\
54.204.8.151	&	2614	&	\red{x}	&	35994	&	407	&	80\%	&	CN	&	85	&	78\%	\\
37.1.211.206	&	1643	&	\red{x}	&	8025	&	336	&	-	&	DE	&	69	&	74\%	\\
204.13.162.116	&	1520	&	\red{x}	&	35204	&	315	&	60\%	&	XK	&	41	&	76\%	\\
23.94.73.91	&	1506	&	\red{x}	&	61400	&	287	&	13\%	&	UA	&	37	&	57\%	\\
62.76.103.211	&	1489	&	\red{x}	&	6762	&	247	&	85\%	&	RU	&	34	&	47\%	\\
178.32.131.253	&	1416	&	\red{x}	&	3257	&	218	&	80\%	&	FR	&	31	&	70\%	\\
119.1.109.72	&	1340	&	\red{x}	&	5536	&	216	&	61\%	&	FJ	&	28	&	54\%	\\
178.32.131.186	&	1339	&	\red{x}	&	11368	&	210	&	-	&	NA	&	27	&	52\%	\\
54.225.195.235	&	1335	&	\red{x}	&	34040	&	207	&	-	&	GB	&	23	&	58\%	\\
\bottomrule
\end{tabular}
\caption{Severity analysis of Top 10 IPs, ASes, and Countries.}
\label{tab:severity:analysis}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Survivability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Survivability Analysis}

%\ik{@Ikram or @Beri, Motivate and cite the PETS'17 on Survival Analysis of censorship analysis via Kaplan Meier estimator.}

%We leverage the python library "Lifelines" to perform the fitting. It can be said that the importance of this model comes from it's ability to fit censored or unknown information about a target's death. Which is why we must consider how to define the Censored Event, In Figures \ref{Fig:results:survive_hosts} and \ref{Fig:results:survive_attacks} we have defined the censored even to be if the host or is still observed to be malicious during the last time block we have collected (Early 2017). Due to the disproportionate amount of non-censored events as compared to censored events, there is almost no uncertainty within fitted curve for some curves. And as apart of the function, without uncertainty we end up containing the same information as an empirical distribution of lifetimes.

In our measurement, we added entries based on blacklists that we collected overtime. These lists have a different timespan and hence cover different and sometime overlapping periods. As the observation window varies, the data is considered \textit{censored} from a statistic view point. A common way to deal with such data is \textit{survival analysis}, for which
we use the Kaplan-Meier (KM) estimator~\cite{KM}.    

The survival function $S(t)$ represents the probability that a malicious actor is still alive after time $t$. Accordingly, we define the random variable $T$ as the time between the first and the last reported malicious activity. With $F(t)$ 
the cumulative distribution function (CDF) of $T$, the survival function is defined as follows:
$$
S(t) = Pr[T > t] = 1 - F(t)
$$
%Survival Analysis is typically used in Medical Inferencing, to model the longevity of patients within a community. We aim to determine the longevity of malicious activities and participating hosts in our dataset. To this end, we leverage the Kaplan-Meiler (KM) estimator [\red{ref}] \ben{cite paper with use of KM, or original definition?} from the python library {\tt Lifelines}\footnote{https://lifelines.readthedocs.io/} to perform our analysis. We choose the KM estimator model because it provides means to estimate ``censored'' or ``missing'' information of an entity's possible ``death''. We define the censored or missing death event as the host that is still observed to be malicious during the last time-bin (i.e., day, week, or month) that we have collected (Early 2017). 
%\ben{THIS IS A COMMENT ABOUT THE SUITABILITY OF KM (MAYBE DISCUSSION STUFF) Due to the disproportionate amount of known events as compared to censored events, there is almost no uncertainty within fitted curve for some hosts e.g. IP. The final curves, without uncertainty, end up containing the same information as an empirical distribution of lifetimes (CDF). So we must consider how we can define the Censored event here to make this a bit more interesting, additionally the aforementioned Figures have used the Final-Initial Definition of a lifetime, but we can additionally make this more interesting by taking either: }
%\begin{itemize}
%	\item Mean Lifetime (As defined by our Churn Model) for every host
%	\item Lifetimes of all hosts (As defined by our Churn Model), with no averaging/aggregation by host.
%\end{itemize}
%\ben{End Comment}

\begin{figure}[ht!]
\centering
\subfloat[\small Hosts]{\includegraphics[width=0.47\columnwidth]{new_plots/Host_KM_estimate.pdf}
\label{Fig:results:survive_hosts}}
\subfloat[\small Classes of malicious activities]{\includegraphics[width=0.47\columnwidth]{new_plots/Attack_KM_estimate.pdf}\label{Fig:results:survive_attacks}}
\hspace{-0.3cm}
\caption{Survivability analysis: Kaplan-Meier Curve Fit for IPs, ASes, and Countries (Figure~\ref{Fig:results:survive_hosts}) and classes of malicious activities (Figure~\ref{Fig:results:survive_attacks}).} 
\label{vt:survivability:analysis}
\end{figure}  
  


%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{new_plots/Host_KM_estimate.pdf}
%\caption{Kaplan-Meier Curve Fit for Host Survivability. Here is CC[s] represents countries. \beri{What is the confidence intervals? 95 98 99?} \ben{The default 5\% Uncertainty is used}} 
%\label{Fig:results:survive_hosts}
%\end{figure}
 
Figure~\ref{Fig:results:survive_hosts} depicts $S(t)$ for IP, ASN and country with a confidence interval of 95\%. First, we observe that our estimator has a very low uncertainty for both IPs and ASN and medium one for country. This is mainly due to the number of data points for each category. Second, we observe the same pattern for \textit{micro vs macro} behavior: IP hosts tend to be one time offenders with 87\% having only \red{one?} day of survivability while this number drastically decreases for both ASN and country with 69\%, 29\% respectively. Finally, it is worth noting that while $S(t)$ tends to zero for both IP and ASN, ~25\% of country population still alive after our observation period \beri{why?}.
\beriw{Same conclusion as above. Findings expected. We need more here if possible}
     
%In Figure~\ref{Fig:results:survive_hosts} we present our survivability analysis of Hosts. We observe the uncertainty bounds around the different tiers of infrastructure. As the countries set has less unique entries within it's set, for the countries which have been marked as having a missing death event is proportionally larger, it therefore has a larger uncertainty bound for it's estimates. Similarly, for IPs however as there is such a large number of unique IPs the relatively low number of censored IPs have little effect and the KM model indicated with certainty the distribution of the survival. Finally, we can observe clearly that amount of One time offenders within the dataset by observing the y-intercepts of these curves. For IP,ASN,CC we have 87\%, 69\%, 29\% respectively.  Another thing to note is that the CC's have a portion ~25\% that are continuing to survive according to this KM estimator, unlike with the ASN and IP estimates they approach 0, This continually surviving proportion of CC's indicate that the lifetime of a given country is likely to continue beyond 3500 days, the length of our dataset.

%\begin{figure}[ht!]
%\centering
%\includegraphics[width=1\columnwidth]{new_plots/Attack_KM_estimate.pdf}
%\caption{Survivability Analysis: Kaplan-Meier Curve Fit for classes of malicious activities. \ben{Will change colors to match the existing malicious activities scheme from earlier}} 
%\label{Fig:results:survive_attacks}
%\end{figure}

Next, we perform Hosts survivability analysis for hosts that correspond to different malicious activities. We are interested to determine whether certain hosts (if any) in a specific class survive longer than the other. We show the results of our analysis in Figure~\ref{Fig:results:survive_attacks}. Observe no significant differences among different classes of malicious activities. Unlike countries survivability trend in Figure~\ref{Fig:results:survive_hosts}, the long tails of the curves suggest that the classes of malicious activities have less likely to have persistent long-term malicious hosts. We can observe that Unwanted programs have the highest likelihood of survivability.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Degree - Lifetime
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Lifetime Attack Type Participation}

\subsection{Hosts' Lifetime and Activity Diversity Analysis}
%Malicious Activities Class Participation}
%\ben{Formerly Degree-Lifetime, might be able to aggregate under the same heading as Entropy: Host - Attack}

\begin{figure*}[ht!]
\centering
\subfloat[\small Malicious IPs]{\includegraphics[width=0.33\textwidth]{new_plots/ip_degree_lifetime.pdf}\label{Fig:results:asn_degree_by_time}}
\subfloat[\small Malicious \textit{ASNs}.]{\includegraphics[width=0.33\textwidth]{new_plots/asn_degree_lifetime.pdf}\label{Fig:results:asn_degree_by_time}}
\subfloat[\small Malicious \textit{Countries}.]{\includegraphics[width=0.33\textwidth]{new_plots/cc_degree_lifetime.pdf}\label{Fig:results:cc_degree_by_time}}
\hspace{-0.3cm}
\caption{IPs, ASNs, and Countries specialization and Lifetime analysis. } 
\label{vt:lifecycle_specialization:analysis}
\end{figure*}

%This Section will now investigate the relationship between the Time Active (The time difference from the first time it was seen to be active, to the last time it was seen active) and the Degree Distribution (The number of attacks the host has contributed to). 
In this Section, we aim to find (if any) relationship between lifetime and diversity of malicious activities of an IP (resp. AS and Country). 

Figures \ref{Fig:results:asn_degree_by_time} highlights the cumulative distribution of the infrastructure components' lifetimes, for the different different numbers of malicious activities they have participated in.

Next, we analyze the specialization of countries in our dataset. We present our analysis in Figure~\ref{Fig:results:cc_degree_by_time}. We observe in the CDF and in the changing colors of the Scatter that there is a clear relationship between the longevity of the malicious tier of infrastructure and the Degree (the number of attacks if participates within), This confirms what can be thought as a straightforward conclusion. In the countries (CC) plot we can note that within the single attack offenders, 46\% are also one time offenders, as they do not have a lifetime greater than 0 days. With any country CC of higher than 1 degree there are no one-time offenders (i.e., Host such as IP, ASN, or Country), we can speculate that this may be a result that attacks may not occur simultaneously within the same time periods. \ik{more info on 'concurrency' of activities.}

It is noted that we do not consider differences between attack classes in the degree (e.g. Malware and Phishing by one Host, compared to another contributing Exploits and Spamming will both be regarded as having degree 2)


%Note: Scatter Plot y-axis has no meaning and something else can be substituted in for meaning.

%Note: Scatter Plot cannot be produced for IPs as there are too many points within the scatter plot to render, But CDF can be.

%Note: Observe the scatter plot changing colors as you progress down the Time(Days) axis, this is inline with what is being observed within the CDF



%\begin{figure}[ht!]
%\centering
%\subfloat[\small Malicious \textit{ASNs} on intervals of Lifecycle.]{\includegraphics[width=1\columnwidth]{./plots/eplots/ASN_SwarmPlot_good.pdf}\label{Fig:results:asn_degree_by_time}}\quad
%\subfloat[\small Malicious \textit{Countries} on intervals of Lifecycle]{\includegraphics[width=1\columnwidth]{./plots/eplots/CC_SwarmPlot.pdf}\label{Fig:results:cc_degree_by_time}}
%\hspace{-0.3cm}
%\caption{Hosts' specialization and Lifetime analysis. } 
%\label{vt:lifecycle_specialization:analysis}
%\end{figure}

%\begin{figure}[t!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/ASN_SwarmPlot_good.pdf}
%\caption{Time Analysis: CDF of malicious \textit{ASNs} on intervals of Lifecycle.  \ben{See Figure \ref{Fig:results:cc_degree_by_time}, as it follows a similar train of reasoning.} }
%\label{Fig:results:asn_degree_by_time}
%\end{figure}


%\begin{figure}[t!]
%\centering
%\includegraphics[width=1\columnwidth]{./plots/eplots/CC_SwarmPlot.pdf}
%\caption{Time Analysis: CDF of malicious \textit{Countries} on intervals of Lifecycle. }} 
%\label{Fig:results:cc_degree_by_time}
%\end{figure}

%\ik{@Ben, push all your analysis methodology and figures in here.}
%\section{Case Study and Current State}
%\begin{enumerate}
%\item Analyze the VirusTotal reports for all domains/URLs/IPs reported in the attacks. 
%\item Case study of at least two prominent attacks, specific malware e.g., Mriai or phishing attack.
%\end{enumerate}

